Unsteady aerodynamics of porous aerofoils

We extend unsteady thin aerofoil theory to model aerofoils with generalised chordwise porosity distributions. The analysis considers a linearised porosity boundary condition where the seepage velocity through the aerofoil is related to the local pressure jump across the aerofoil surface and to the unsteady characteristics of the porous medium. Application of the Plemelj formulae to the resulting boundary value problem yields a singular Fredholm--Volterra integral equation which does not admit an analytic solution. Accordingly, we develop a numerical solution scheme by expanding the bound vorticity distribution in terms of appropriate basis functions. Asymptotic analysis at the leading- and trailing-edges reveals that the appropriate basis functions are weighted Jacobi polynomials whose parameters are related to the porosity distribution. The Jacobi polynomial basis enables the construction of a numerical scheme that is accurate and rapid, in contrast to the standard choice of Chebyshev basis functions that are shown to {be unsuitable} for porous aerofoils. Applications of the numerical solution scheme to discontinuous porosity profiles, quasi-static problems, and the separation of circulatory and non-circulatory contributions are presented. Analogues to the classical Theodorsen and Sears functions are computed numerically, which show that an effect of trailing-edge porosity is to reduce the amount of vorticity shed into the wake, thereby reducing the magnitude of the circulatory lift. {Fourier transform inversion of these frequency-domain functions produces porous extensions to the Wagner and K\"{u}ssner functions for transient aerofoil motions or gust encounters, respectively.}

==> sections/Mathematical_Method.tex <==
\section{Mathematical model}\label{MM}
Consider a thin airfoil undergoing prescribed unsteady motions in a two-dimensional steady, incompressible flow. Supposing a chord length $l$, mean flow speed $U$, and fluid density $\rho$, all terms are nondimensionalized using $l$, $l/U$, and $\frac{1}{2} \rho U^2$ as the length, time, and pressure scales, respectively. 




\subsection{Porous boundary condition}
Along a porous airfoil, the perturbation flow velocity on the wing surface, $w$, is related to the local seepage flow rate directed along the unit normal to the panel surface, $w_s$, as the following
\begin{eqnarray}\label{w01}
w(x,t)=w_s+\frac{\partial z_a}{\partial x}+\frac{\partial z_a}{\partial t},
\end{eqnarray}
where the function $z_a(x,t)$ defines the mean surface of the airfoil.


For an airfoil with a Darcy-type porosity distribution under conditions that permit omission of nonlinear flow and acoustic effects (cf.~\cite{nayfeh1975acoustics, bauer1977impedance, jordan2005growth}), the local flow rate is linearly proportional to the porosity and the pressure distribution across the porous medium \cite{Rus,HJ}:
\begin{equation}\label{ws}
w_s=\frac{1}{2}\delta R(x) \Delta p(x,t).
\end{equation} 
%
Here, $\delta=\rho U C$ is the dimensionless porosity parameter \cite{HJ}, $C$ is the porosity coefficient, $R(x)$ is a dimensionless function defining the porosity distribution, and $\Delta p(x,t)$ is the dimensionless pressure jump (lower minus upper) across the airfoil. Comparison of the relationship between the local pressure jump $\Delta p$ and seepage velocity $w_s$ against the standard Darcy boundary condition~\cite{BSL} allows the product $C R(x)$ to be defined in terms of physical parameters:
%
\begin{equation}
    C R(x)=\frac{\kappa}{\mu d}.
\end{equation}
%
The symbol $\mu$ denotes the fluid viscosity, $\kappa$, and $d$ represent the permeability, and thickness of the porous material, respectively, all which may vary with chordwise location $x$.  

\subsection{Derivation of the singular integral equation}
The pressure jump across the airfoil can be expressed entirely in terms of the circulation on the wing $\gamma_a$ (Eq.~(5-321) in \cite{A}). This permits Eq.~(\ref{ws}) to be written in the following 
\begin{eqnarray}\label{ws-new}
w_s&=&\delta R(x) \left(\gamma_a+\frac{\partial}{\partial t}\int_{-1}^x \gamma_a d\xi \right).
\end{eqnarray}

On the other hand, $w$ is related to the running circulations on the wing, $\gamma_a$, and on the wake, $\gamma_w$ through the following integral equation: \begin{equation}\label{ww}
   w(x,t)= \frac{1}{2\pi}\dashint_{-1}^{1}\frac{\gamma_a(\xi,t)}{\xi-x}d\xi +\frac{1}{2\pi}\int_{1}^{\infty}\frac{\gamma_w(\xi,t)}{\xi-x} d\xi.
\end{equation}
Substitution of Eqs.~(\ref{ws-new},\ref{ww}) into the Eq.~(\ref{w01}) furnishes the following singular integral equation for the circulations on the airfoil and into the wake:
\begin{align}\label{p_unsteady}
\delta R(x) \left[\gamma_a(x,t) + \frac{\partial}{\partial t} \int_{-1}^x \gamma_a(\xi,t) d\xi \right]& \notag\\
-\frac{1}{2\pi}\dashint_{-1}^{1}\frac{\gamma_a(\xi,t)}{\xi-x}d\xi &-\frac{1}{2\pi}\int_{1}^{\infty}\frac{\gamma_w(\xi,t)}{\xi-x} d\xi=- \left( \frac{\partial z_a}{\partial t} + \frac{\partial z_a}{\partial x}   \right).
\end{align}

==> sections/chebyshev-comparison.tex <==
\section{Comparison to Chebyshev expansion}

In this section we compare the solution to an expansion in terms of Chebyshev polynomials, such as in \eqref{Eq:ChebRig}. We define the error as 

There are several issues with this expansion which will be illustrated below.

For example, the above expansion will give spurious results for the leading edge suction force.

We now explore the error compared to exact solutions for the steady case.

\begin{align}
    \epsilon &= \int_{-1}^{1} 
\end{align}

==> sections/circ.tex <==

\subsection{Circulatory unsteady solution}
%
The circulatory part satisfies
%
\begin{align}
\mathcal{L} \left[\vortNC\right](x)&=f_C(x)
 \label{Eq:SVCcirc}
\end{align}
%
We note that we may $f_C$ as
    %
    \begin{align*}
    \int_1^{\infty} \frac{\e^{\i k \xi}}{\xi - x} \d \xi = \e^{\i k x}\Gamma(0,\i k (x-1))
    \end{align*}
    %
    where
    %
    \begin{align*}
    \Gamma(s,z)&= \int_{z}^{\infty} t^{s-1}{\e^{-t}} \d t.
    \end{align*}
    %
is the incomplete Gamma function. Accordingly, we obtain the asymptotic behaviour
    %
    \begin{align*}
    f_C(x) \sim -\e^{\i k} \left(E - \frac{\i \pi}{2} + \log(k(1-x)) \right), \qquad \qquad \textrm{as } x \rightarrow 1,
    \end{align*}
    %
    where $E$ is the Euler–Mascheroni constant.

We now seek an ansatz of the form
%
\begin{align*}
\vortC(x) &= \frac{\left((1-x)^\alpha f(x)+c\right)}{(1+x)^\beta}.
\end{align*}
%
where $f$ is a smooth function and $c$ is a constant.
%    
Consequently, using the typical ansatz we again have the following asymptotic behaviours in \eqref{Eq:SVCcirc} as $x \rightarrow -1$,
%
\begin{align*}
\vortC(x) &\sim \frac{\left(2^\alpha f(-1) + c \right)}{(1+x)^\beta}, \\
\int_{-1}^x \vortC(\xi) \d \xi &\sim 0, \\
\frac{1}{\pi}\dashint_{-1}^1 \frac{\vortC(\xi)}{\xi - x} \d \xi & \sim \frac{\cot(\beta \pi)}{(1+x)^\beta}\left( 2^\alpha f(-1) + c \right), \\
 \frac{- \i \helmNum}{\pi}\int_{1}^{\infty}\frac{\e^{\i \helmNum \xi}}{\xi-x} \d \xi &\sim   \frac{- \i k}{\pi} \Gamma(0,-2 \i k ).
\end{align*}
%
Accordingly, by cancelling the leading-order singularity we again obtain 
%
\begin{align*}
\beta = \frac{1}{\pi} \cot^{-1} \psi(-1).
\end{align*}
%
We now apply the same procedure at the trailing-edge. We now have, as $x \rightarrow 1$,
%
\begin{align*}
\vortC(x) &\sim \frac{\left((1-x)^\alpha f(1) + c \right)}{2^\beta}, \\
\int_{-1}^x \vortC(\xi) \d \xi &\sim \int_{-1}^1 \vortC(\xi) \d \xi, \\
\frac{1}{\pi}\dashint_{-1}^1 \frac{\vortC(\xi)}{\xi - x} \d \xi & \sim \frac{1}{\pi}\dashint_{-1}^1 \frac{\vortC(\xi)}{\xi - 1} \d \xi + (1-x)^\alpha\frac{\cot(\alpha \pi) f(1)}{2^\beta} + \log(x-1)\frac{c}{\pi 2^\beta} , \\
 \frac{- \i \helmNum}{\pi}\int_{1}^{\infty}\frac{\e^{\i \helmNum \xi}}{\xi-x} \d \xi &\sim \frac{\i k }{\pi} \e^{\i k} \left(\gamma - \frac{\i \pi}{2} + \log(k) + \log(1-x) \right) 
\end{align*}
%
Accordingly, we identify 
%
\begin{align*}
c &= -2^\beta\i k \e^{\i k},\\
\beta &= \frac{1}{\pi} \cot^{-1} \psi(1).
\end{align*}
%
Consequently, we write
%
\begin{align*}
\vortC(x) &= \frac{(1-x)^\alpha}{(1+x)^\beta}\vortCCoefs{0} + (1-x)^\alpha(1+x)^{1-\beta} \sum_{n=1}^\infty \vortCCoefs{n} P^{\alpha,1-\beta}_{n-1}(x) + \frac{c}{(1+x)^\beta}
\end{align*}
%

Note that 
%
\begin{align*}
\mathcal{L}\left[\frac{1}{(1+x)^\beta}\right](x) &= \psi(x)\left[\frac{1}{(1+x)^\beta} + \i k \frac{(1+x)^{1- \beta}}{1- \beta}\right] - \frac{1}{\pi} 
\end{align*}
%
 Accordingly, we may apply a similar expansion as in equation \eqref{Eq:JacExpanNC} to obtain the coefficients for the vorticity distribution:
%
 \begin{align}
    \vortC(x) &=  \vortCCoefs{0} \left( \weight{x}{\alpha}{-\beta} - \frac{2 \alpha}{1+ \alpha - \beta} \weight{x}{\alpha-1}{-\beta}\right) \notag \\
    &+\vortCCoefs{1} \left(\weight{x}{\alpha}{1- \beta} - \frac{4 \alpha(1-\beta)}{(1 + \alpha - \beta)(2+ \alpha - \beta)}  \weight{x}{\alpha-1}{-\beta}  \right) \notag  \\
    & + \weight{x}{\alpha}{1-\beta} \sum_{n=2}^\infty \vortCCoefs{n} P_{n-1}^{\alpha,1-\beta} (x)\notag \\
    & +c \left(\weight{x}{0}{-\beta}- 2^{1-\alpha}\frac{B(1-\beta,1)}{B(1-\beta,\alpha)}\weight{x}{\alpha-1}{-\beta} \right) \notag\\
    & + \frac{\weight{x}{\alpha-1}{-\beta}}{2^{\alpha-\beta}B(1- \beta,\alpha)}. \label{Eq:JacExpanC}
\end{align}
%
Consequently, as $x \rightarrow 1$ we have $\gamma_C(x) \sim  \Lambda_C (1-x)^{\alpha-1}$ where
%
\begin{align*}
\Lambda_C = -2^{-\beta} \left( \frac{  \vortCCoefs{0}2 \alpha}{1+ \alpha - \beta} +\frac{ \vortCCoefs{1} 4 \alpha(1-\beta)}{(1 + \alpha - \beta)(2+ \alpha - \beta)} + \frac{ 2 c B(1-\beta,1) - 2^{\beta}}{2^\alpha B(1- \beta,\alpha)} \right).
\end{align*}
%
In order to quicken the collocation scheme, we subtract the singular behaviour from the circulatory vorticity and write
%
\begin{align*}
{\tildVortC}(x) = {\vortC}(x) - \left[c \left(\weight{x}{0}{-\beta}- 2^{1-\alpha}\frac{B(1-\beta,1)}{B(1-\beta,\alpha)}\weight{x}{\alpha-1}{-\beta} \right) + \frac{ \weight{x}{\alpha-1}{-\beta}}{ 2^{\alpha-\beta} B(1- \beta,\alpha)} \right]
\end{align*}
%
satisfies
%
\begin{align*}
\mathcal{L}\left[\tildVortC\right](x) &= f_C(x) - \mathcal{L}\left[\frac{c}{(1+x)^\beta}\right](x)
\end{align*}
%
and the right hand side is now regular as $x\rightarrow \pm 1$.


\subsection{Tuning the circulation}
%
We choose the circulation such that the singularities at the trailing-edge from the circulatory and non-circulatory solutions cancel. In order words, we write
%
\begin{align*}
\wakeStrength = -\frac{\Lambda_N}{\Lambda_C}.
\end{align*}
%
This ensures that the Kutta condition is satisfied.

==> sections/continuous-porosity.tex <==
\subsection{Solution for aerofoils with continuous porosity distributions}

 This is permissible for the rigid aerofoil case, where the end point behaviour is known to be $(1\pm x)^{\mp 1/2}$ at the leading and trailing edges respectively. However, in our case, this behaviour is not given. In fact, it was shown in \cite{A} that one of the effects of porosity is to vary the strength of a singularity or zero at the edges. Consequently, the expansion of \eqref{Eq:ChebRig} is not appropriate. Therefore, we write the pressure in the form
%
\begin{align}
    p(x) =\frac{(1-x)^\alpha}{(1+x)^\beta} \cdot p^\ast(x), \label{Eq:presExp1}
\end{align}
%
where $p^\ast(x)$ is a function that is H\"older continuous on $[-1,1]$ and is non-zero at $x=1$. Substituting this expression into our singular integral equation \eqref{p_steady} yields
%
\begin{equation}\label{p_steady2}
\rho UC R(x)\frac{(1-x)^\alpha}{(1+x)^\beta} \cdot p^\ast(x)-\frac{1}{2\pi}\dashint_{-1}^{1} \frac{(1-t)^\alpha}{(1+t)^\beta} \cdot \frac{p^\ast(t)}{t-x}dt~=~2\frac{dz}{dx}.
\end{equation}
%
The next step is to determine $\alpha$ and $\beta$, which represent the intensity of the zero/singularity at the trailing/leading edge. We first investigate the behaviour at the trailing edge. If we let $x \rightarrow -1$ and apply \eqref{Eq:LEAsymptotics}, our singular integral equation \eqref{p_steady2} becomes, at leading order,
%
\begin{align*}
    \rho U C R(-1) \frac{2^{\alpha}}{(1+x)^\beta} p^\ast(-1) + \frac{\cot\left(\beta \pi\right)}{2} \cdot \frac{2^{\alpha}}{(1+x)^\beta} &=0
\end{align*}
%
and therefore we obtain
%
\begin{align*}
  \beta = \frac{1}{\pi}\cot^{-1} \left( - 2 \rho U C R(-1)  \right).
\end{align*}
%
Applying a similar approach at the trailing edge and employing \eqref{Eq:TEAsymptotics} gives, at leading order,
%
\begin{align*}
    \rho U C R(1) \frac{(1-t)^{\alpha}}{2^\beta} p^\ast(1) -\i A(1) - \i \Phi_0(1) + \frac{(1- t)^\alpha}{2^\beta} p^\ast(1) \cdot \cot(\alpha \pi) &= 2 \frac{\d z}{\d x}.
\end{align*}

The above must match at every order. By matching $(1-t)^\alpha$ terms, we obtain

\begin{align*}
  \alpha = \frac{1}{\pi}\cot^{-1} \left(- 2 \rho U C R(1)  \right).
\end{align*}

Considering a constant porosity distribution recovers the results of \cite{A}.

This informs us to expand the pressure into a series of Jacobi polynomials in a similar way to Rienstra (1992)

\begin{align}
    p(x) = p_0 \frac{(1-x)^\alpha}{(1+x)^\beta} + (1-x)^\alpha(1+x)^\beta \sum_{n=1}^\infty p_n P_{n-1}^{\alpha,\beta} (x). \label{Eq:JacExpan}
\end{align}

where $P_n^{\alpha,\beta}$ represents the $n^{th}$ Jacobi polynomial which has weight function $\weight{x}{\alpha}{\beta} \coloneqq (1-x)^\alpha(1+x)^\beta $. 

We may now substitute our Jacobi polynomials expansion \eqref{Eq:JacExpan} into our singular integral equation \eqref{p_steady}. Applying \eqref{Eq:JacobiHilbertTransform} to \eqref{p_steady} yields 

\begin{align}\nonumber
    &\rho UC R(x)\left(p_0 \weight{x}{\alpha}{-\beta}+ \weight{x}{\alpha}{\beta} \sum_{n=1}^\infty p_n P_{n-1}^{\alpha,\beta} (x)  \right) \\
    &- \frac{1}{2 \pi} \left( p_0 \weight{x}{\alpha}{-\beta} Q_0^{\alpha,-\beta}(x) + \weight{x}{\alpha}{\beta} \sum_{n=1}^\infty p_n  Q_{n-1}^{\alpha,\beta} (x) \right) =~2\frac{dz}{dx},
\end{align}

or alternatively,

\begin{align} \label{Eq:presCoef1}
    p_0 f_0^{\alpha,-\beta}(x) + \sum_{n=1}^\infty p_n f_{n-1}^{\alpha,\beta} (x)  =~4\frac{dz}{dx},
\end{align}

where

\begin{align*}
    f_n^{\alpha,\beta}(x) &= \weight{x}{\alpha}{\beta} \left( \psi(x) P_n^{\alpha, \beta}(x) - \frac{1}{\pi} Q_n^{\alpha,\beta}(x) \right) .
\end{align*}

We may follow the approach of Rienstra (1992) and expand the right hand side in Chebyshev polynomials. Any expansion in orthogonal polynomials is valid, but we choose the Chebyshev polynomials of the second kind in order to be consistent with Rienstra (1992). Therefore \eqref{Eq:presCoef1} becomes

\begin{align}
    p_0  f_0^{\alpha,-\beta}(x) + \sum_{n=1}^\infty p_n f_{n-1}^{\alpha,\beta} (x) = 4 \sum_{n=1}^\infty v_n U_{n-1}(x).
\end{align}

Consequently, we may obtain a system of equations for the $p_n$ by multiplying by $U_{m-1}(x) \cdot \weight{x}{\frac{1}{2}}{\frac{1}{2}}$ for $m=1 \dots M$ and integrating from $-1$ to $1$:

\begin{align}
    p_0 F_{0,m}^{\alpha,-\beta} + \sum_{n=1}^\infty p_n F_{n,m} = 2 v_{m-1} \pi,
\end{align}

where 

\begin{align}
    F_{n,m}^{\alpha,\beta} &=
    \begin{dcases}\int_{-1}^1 \weight{x}{\frac{1}{2}}{\frac{1}{2}} \cdot f_{n-1}^{\alpha,\beta}(x) \cdot U_{m-1}(x) \d x & n> 0, \\
   \int_{-1}^1 \weight{x}{\frac{1}{2}}{\frac{1}{2}} \cdot f_{0}^{\alpha,-\beta}(x) \cdot U_{m-1}(x) \d x  & n =0.
    \end{dcases} \label{Eq:SteadyFDef}
\end{align}

In matrix form we write

\begin{align*}
   \boldsymbol{F} \boldsymbol{p} = 2 \pi \boldsymbol{v},
\end{align*}

so that 

\begin{align*}
  \boldsymbol{p} = 2 \pi  \boldsymbol{F}^{-1} \boldsymbol{v}.
\end{align*}


==> sections/define-colours.tex <==
\usepackage{xcolor}
\usepackage{colortbl}

\definecolor{themecolour}{rgb}{0.64, 0.76, 0.68}
\definecolor{mygray}{rgb}{0.7, 0.7, 0.7}
\definecolor{tablegray}{rgb}{0.75, 0.75, 0.75}
\definecolor{confcol}{RGB}{255, 255, 255}
\definecolor{camblue}{RGB}{108, 172, 228}
\definecolor{camred}{RGB}{213, 0, 50}
\definecolor{camnavy}{RGB}{0, 60, 113}
\definecolor{camgreen}{RGB}{114, 180, 49}

\definecolor{myblue}{rgb}{0 ,  0.4470 , 0.7410}
\definecolor{myorange}{rgb}{0.8500,    0.3250,    0.0980}
\definecolor{myyellow}{rgb}{0.9290,    0.6940,    0.1250}
\definecolor{mypurple}{rgb}{ 0.4940,    0.1840,    0.5560}
\definecolor{myred}{rgb}{     0.6350 ,   0.0780 ,   0.1840}
\definecolor{mygreen}{rgb}{         0.4660  ,  0.6740   , 0.1880}

\definecolor{branchCol}{rgb}{0, .8, .8}

\definecolor{prsared}{RGB}{ 219,25,73}
\definecolor{prsablue}{RGB}{ 4,146,210}

\definecolor{confblue}{rgb}{0.75, 0.72, 0.95}
\definecolor{confgreen}{rgb}{0.76, 1, 0.74}
\definecolor{confgrey}{rgb}{0.9, .9, 0.9}

\definecolor{cvblue}{rgb}{0.22,0.45,0.70}% light blue

\definecolor{matlab1}{rgb}{0,0.4470,0.7410}
\definecolor{matlab2}{rgb}{0.8500,0.3250,0.0980}
\definecolor{matlab3}{rgb}{0.9290,0.6940,0.0980}
\definecolor{matlab4}{rgb}{0.4940,0.1840,0.5560}
\definecolor{matlab5}{rgb}{0.4660,0.6740,0.1880}
\definecolor{matlab6}{rgb}{0.3010,0.7450,0.9330}
\definecolor{matlab7}{rgb}{0.6350,0.0780,0.1840}

==> sections/non-circ.tex <==
\subsection{Unsteady non-circulatory solution}
%
The non-circulatory part satisfies
%
\begin{align}
\mathcal{L} \left[\vortNC\right](x) &=f_N(x),% \tag{\theequation.a} 
\label{Eq:SVFncirc}
\end{align}
%
in addition to 
%
\begin{align}
\int_{-1}^1 \vortNC(\xi) \d \xi = 0. \label{Eq:zeroCirc}
\end{align}
%
However, it is not possible to enforce the zero-circulation condition \eqref{Eq:zeroCirc} in addition to the Kutta condition at the trailing-edge. Accordingly, we follow \cite{A} and relax the Kutta condition in the non-circulatory part in order to enforce \eqref{Eq:zeroCirc}. Practically speaking, we do not enforce that $\vortNC(\xi)$ vanishes as $\xi \rightarrow 1$. Following the previous sections, we seek a solution of \eqref{Eq:SVFncirc} of the form
%
\begin{align*}
\vortNC(x) &= \frac{(1-x)^\alpha}{(1+x)^\beta}f(x),
\end{align*}
%
where $f$ is a smooth function. We now note that, as $x\rightarrow -1$
%
\begin{align*}
\vortNC(x) &\sim \frac{2^\alpha}{(1+x)^\beta}f(-1), \\
\int_{-1}^x \vortNC(\xi) \d \xi &\sim 0, \\
\frac{1}{\pi}\dashint_{-1}^1 \frac{\vortNC(\xi)}{\xi - x} \d \xi & \sim 2^{\alpha}\frac{\cot(\beta \pi)}{(1+x)^\beta}f(-1), \\
 \frac{\partial z_a}{\partial t}(x) + \frac{\partial z_a}{\partial x}(x) &\sim    \frac{\partial z_a}{\partial t}(-1) + \frac{\partial z_a}{\partial x}(-1).
\end{align*}
%
Consequently, for terms for match at leading-order, we require
%
\begin{align*}
2^\alpha \frac{\psi(-1)}{(1+x)^\beta}f(-1) -2^{\alpha}\frac{\cot(\beta \pi)}{(1+x)^\beta}f(-1)=0,
\end{align*}
%
i.e. 
%
\begin{align*}
\beta = \frac{1}{\pi} \cot^{-1}(\psi(-1)) + n,
\end{align*}
%
for $n \in \mathbb{Z}$.
We now inspect the behaviour as $x \rightarrow 1$. In this case, we have
%
\begin{align*}
\vortNC(x) &\sim \frac{(1-x)^\alpha}{2^\beta}f(1), \\
\int_{-1}^x \vortNC(\xi) \d \xi &\sim \int_{-1}^1 \vortNC(\xi) \d \xi, \\
\frac{1}{\pi}\dashint_{-1}^1 \frac{\vortNC(\xi)}{\xi - x} \d \xi & \sim \frac{1}{\pi}\dashint_{-1}^1 \frac{\vortNC(\xi)}{\xi - 1} \d \xi -\frac{\cot(\alpha \pi)}{2^\beta}(1-x)^\alpha f(1), \\
 \frac{\partial z_a}{\partial t}(x) + \frac{\partial z_a}{\partial x}(x) &\sim  \frac{\partial z_a}{\partial t}(-1) + \frac{\partial z_a}{\partial x}(1).
\end{align*}
%
Similarly, we get 
%
\begin{align*}
\alpha = \frac{1}{\pi} \cot^{-1}(\psi(1)) + n,
\end{align*}
%
for $n \in \mathbb{Z}$. In a similar way to section \ref{Sec:Steady}, we seek an expansion of the non-circulatory vorticity distribution of the form
%
 \begin{align}
    \vortNC(x) &=  \vortNCCoefs{0} \left( \weight{x}{\alpha}{-\beta} - \frac{2 \alpha}{1+ \alpha - \beta} \weight{x}{\alpha-1}{-\beta}\right) \notag \\
    &+\vortNCCoefs{1} \left(\weight{x}{\alpha}{1- \beta} - \frac{4 \alpha(1-\beta)}{(1 + \alpha - \beta)(2+ \alpha - \beta)}  \weight{x}{\alpha-1}{-\beta}  \right) \notag  \\
    & + \weight{x}{\alpha}{1-\beta} \sum_{n=2}^\infty \vortNCCoefs{n} P_{n-1}^{\alpha,1-\beta} (x) \label{Eq:JacExpanNC}
\end{align}
%
so that \eqref{Eq:zeroCirc} is automatically satisfied. Consequently, as $x \rightarrow 1$ we have $\vortNC(x) \sim  \Lambda_N (1-x)^{\alpha-1}$ where
%
\begin{align*}
\Lambda_N = -2^{-\beta} \left( \frac{  \vortNCCoefs{0}2 \alpha}{1+ \alpha - \beta} +\frac{ \vortNCCoefs{1} 4 \alpha(1-\beta)}{(1 + \alpha - \beta)(2+ \alpha - \beta)} \right).
\end{align*}
%
We may use \eqref{Eq:WeightedJacobiIntegral} to write
%
\begin{align*}
\int_{-1}^x\vortNC(\xi) \d \xi & = \vortNCCoefs{0} \left( 2^{1+\alpha-\beta}B\left(\frac{1+x}{2};1-\beta,1+\alpha\right) \right) + \vortNCCoefs{1} \left(2^{2+\alpha-\beta}B\left(\frac{1+x}{2};2-\beta,1+\alpha\right) \right)\\
& - \sum_{n=2}^\infty \frac{\vortNCCoefs{n}}{2(n-1)} \weight{x}{\alpha+1}{2-\beta} P_{n-2}^{\alpha+1,2-\beta} (x).
\end{align*}
%
Consequently, we may express \eqref{Eq:SVFncirc} as
%
\begin{align*}
\sum_{n=0}^\infty \vortNCCoefs{n} f_n^{\alpha,\beta}(x) &= f_N(x)
\end{align*}
%
where
%
\begin{align*}
f_0^{\alpha,\beta}(x) & = \psi(x)\left\{1 + \i k I_0^{\alpha,-\beta}(x) \right\} -\frac{1}{\pi} \weight{x}{\alpha}{-\beta}Q_0^{\alpha,-\beta}(x),  \\
f_n^{\alpha,\beta}(x) &= \psi(x)\left\{1 +\i k I_n^{\alpha,1-\beta}(x) \right\}-\frac{1}{\pi} \weight{x}{\alpha}{1-\beta}Q_{n}^{\alpha,1-\beta}(x) ,\qquad n>0.\\
\end{align*}
%
We can now collocate and solve the problem.
%

==> sections/partially-porous-steady.tex <==
\subsection{Solution for discontinuous porosity distributions}

We may also use the new method to find the pressure distribution for a partially porous aerofoil. These aerofoils consist of an impermeable forward section and a permeable aft section \cite{gil}. It is generally believed that this aerofoil design possess superior aerodynamic qualities compared to aerofoils that are uniformly porous \cite{gil2,gil,Hajian2017}. We place the permeable-impermeable junction at $x = c$, so that the singular integral equation for a steady, partially porous aerofoil becomes
%
\begin{align}
H(x - c) \psi(x) p(x)-\frac{1}{\pi}\dashint_{-1}^{1}\frac{p(t)}{t-x}\d t=4\frac{\d z}{\d x}(x), \label{Eq:ppGE}
\end{align}
%
where $H(\cdot)$ is the heaviside function, i.e.
%
\begin{align}
    H(x - c) = \begin{cases}
    0, \qquad x<c, \\
    1, \qquad x>c,
    \end{cases}
\end{align}
%
and $\psi(x) = 2 \rho U C R(x)$. We first note that we require $p=0$ at $x = c$, otherwise there would be a discontinuity in the seepage velocity through the wing. Consequently, we write the pressure in the form 
%
\begin{align}
p(x) &= p^\ast(x) (x-c)^\gamma, && p^\ast(x) = \frac{(1-x)^\alpha}{(1+x)^\beta} \e^{\i \pi \gamma H(c-x)} \tilde{p}(x), \label{Eq:pDiscFac}
\end{align}
%
where $\tilde{p}$ is piecewise H\"older continuous. Applying a similar argument to the previous section via analysis of \eqref{Eq:ppGE} at the endpoints yields
%
\begin{align}
\addtocounter{equation}{1}
    \alpha &= \frac{1}{\pi} \cot^{-1} \left(H({+}1-c)\psi({+}1) \right) =  \frac{1}{\pi} \cot^{-1} \left(\psi(1) \right), \tag{\theequation.a} \label{Eq:ppAlphDef}\\
    \beta &= \frac{1}{\pi} \cot^{-1} \left( H(-1-c)\psi(-1) \right) = \frac{1}{2}. \tag{\theequation.b} 
\end{align}
%
We now consider the asymptotic behaviour as $x \rightarrow c^\pm$, where $c^\pm = c \pm 0$. In these limits, note that \eqref{Eq:pDiscFac} yields
%
\begin{align*}
p^\ast(c^-) = \frac{(1-c)^\alpha}{(1+c)^\beta} \e^{\i \pi \gamma} \tilde{p}(c^-), \qquad p^\ast(c^+) = \frac{(1-c)^\alpha}{(1+c)^\beta} \tilde{p}(c^+).
\end{align*}
%
If we substitute \eqref{Eq:pDiscFac} into \eqref{Eq:ppGE} and consider the limit $x \rightarrow c^-$ then we obtain
%
\begin{align}
- \i \left(-\frac{\e^{-\i \gamma \pi} }{2 \i \sin(\gamma \pi)} \frac{(1-c)^\alpha}{(1+c)^\beta} \tilde{p}(c^+) + \frac{\cot(\gamma \pi)}{2 \i } \frac{(1-c)^\alpha}{(1+c)^\beta} \e^{\i \pi \gamma} \tilde{p}(c^-)\right) \cdot \left(x - c\right)^\gamma + C_0+ \Phi_0^{\ast}(x) &= ~4\frac{\d z}{\d x}(c), \label{Eq:pp1}
\end{align}
%
where $C_0$ is a constant, $\Phi_0^\ast(x) = {o}\left((x-c)^\gamma \right)$, and we have used the asymptotic expansions found in \cite{NIM}.

By matching coefficients in \eqref{Eq:pp1}, we see that the coefficient of $(x-c)^\gamma$ must vanish. Consequently, we obtain the identity
%
\begin{align}
\tilde{p}(c^+) =\cos(\gamma \pi)\e^{2 \i \pi \gamma} \tilde{p}(c^-). \label{Eq:ppPJump1}
\end{align}
%
If we now consider $x \rightarrow c ^+$ in \eqref{Eq:ppGE} then we obtain
%
\begin{align*}
\psi(c^+)  \frac{(1-c)^\alpha}{(1+c)^\beta} \tilde{p}(c^+) (x-c)^\gamma +  \i \left(\frac{\e^{\i \gamma \pi}}{2 \i \sin(\gamma \pi)} \frac{(1-c)^\alpha}{(1+c)^\beta} \e^{\i \pi \gamma} \tilde{p}(c^-) - \frac{\cot(\gamma \pi)}{2 \i } \frac{(1-c)^\alpha}{(1+c)^\beta} \tilde{p}(c^+) \right) \cdot \left(x - c\right)^\gamma\\
+ C_1 + \Phi_1^\ast(x) &= 4\frac{\d z}{\d x}(c),
\end{align*}
%
where $C_1$ is a constant and $\Phi_1^\ast(x) = {o}\left((x-c)^\gamma \right)$. Again, the coefficient of $(x-c)^\gamma$ must vanish, i.e.
%
\begin{align}
\psi(c^+) \tilde{p}(c^+) - \i \left(\frac{\e^{\i \gamma \pi}}{2 \i \sin(\gamma \pi)} \e^{\i \pi \gamma} \tilde{p}(c^-) - \frac{\cot(\gamma \pi)}{2 \i } \tilde{p}(c^+) \right)&=0. \label{Eq:ppPJump2}
\end{align}
%
\iffalse
Using \eqref{Eq:ppPJump} we obtain
%
\begin{align*}
\psi(c^+) \cos(\gamma \pi)\e^{2 \i \pi \gamma} \tilde{p}(c^-)+ \i \left(\frac{\e^{\i \gamma \pi}}{2 \i \sin(\gamma \pi)} \e^{\i \pi \gamma} \tilde{p}(c^-) - \frac{\cot(\gamma \pi)}{2 \i } \ \cos(\gamma \pi)\e^{2 \i \pi \gamma} \tilde{p}(c^-) \right)&=0
\end{align*}
%
Rearranging gives
%
\begin{align*}
\psi(c^+) \cos(\gamma \pi)+ \left(\frac{1}{2 \i \sin(\gamma \pi)}  - \frac{\cot(\gamma \pi)}{2 \i }  \cos(\gamma \pi) \right)&=0
\end{align*}
%
which has the solution
\fi
We now combine \eqref{Eq:ppPJump1} and \eqref{Eq:ppPJump2} to obtain
%
\begin{align*}
\gamma &= \frac{1}{\pi} \arctan(\psi(c^+)) = \frac{1}{2} - \frac{1}{\pi} \arccos(\psi(c^+)).
\end{align*}
%
In the case where $R$ is a constant, $\psi(x) \equiv \psi_0$ and \eqref{Eq:pDiscFac} becomes
%
\begin{align}
p(x) & = \left|\frac{ x-c }{ x +1} \right|^{1/2} \cdot \left| \frac{x-1}{x-c} \right|^{\alpha} \tilde{p}(x).
\end{align}
%
Note that the above expression is equivalent to \cite[eq. (13)]{gil2}.
\iffalse
Consequently, we seek solutions of the form

\begin{align*}
p(x) &= \begin{dcases}
p_0^- \frac{(c-x)^{\gamma}}{(1+x)^{1/2} }+ \left(  \frac{4 (x-c)(x+1)}{(c+1)^2} \right)^\gamma \sum_{n=1}^\infty p_n^- P_{n-1}^{\gamma,\gamma} \left( \frac{2 (1+x)}{1+c} -1  \right) & -1 < x \leq c \\
\sqrt{\frac{2}{1-c} } (x-c)^\gamma(1-x)^\alpha\sum_{n=1}^\infty p_n^+ P_{n-1}^{\alpha,\gamma} \left( 1+  \frac{2 (x-1)}{1-c} \right)  & c<x<1
\end{dcases}
\end{align*}
\fi
We now set up the collocation scheme to solve \eqref{Eq:ppGE}. First we use the substitutions
%
\begin{align*}
\tau_1(x) &= -1+2 \frac{x+1}{1+c}, \qquad \qquad -1<x<c,\\
\tau_2(x) &= \phantom{-} 1+ 2 \frac{x-1}{1-c}, \qquad \qquad \phantom{-}c<x<1,
\end{align*}
%
\iffalse
and the equivalent inversions
%
\begin{align*}
x(\tau_1) &= -1+ \frac{(\tau_1+1)(1+c)}{2}, & -1<x<c\\
x(\tau_2) &= \phantom{-} 1+ \frac{(\tau_2-1)(1-c)}{2}, &c<x<1
\end{align*}
%
Note that
%
\begin{align*}
\tau_1 = \phantom{-}1+ (\tau_2+1)\frac{1-c}{1+c}\\
\tau_2 = -1+ (\tau_1-1)\frac{1+c}{1-c}
\end{align*}
%
\fi
so that the integral operator becomes
%
\begin{align*}
\dashint_{-1}^1 \frac{p(t)}{t-x} \d t &= \dashint_{-1}^c  \frac{p_f(t) }{t-x} \d t + \dashint_{c}^1 \frac{ p_a(t)  }{t-x} \d t\\
& = \frac{1+c}{2}  \dashint_{-1}^1   \frac{p_f\left(t(u_1) \right) }{t(u_1)-x} \d u_1 +  \frac{1-c}{2}  \dashint_{-1}^1   \frac{ p_a\left(t(u_2) \right) }{t(u_2)-x} \d u_2 \\
& = \dashint_{-1}^1   \frac{P_f\left(u_1\right) }{u_1-\tau_1(x)} \d u_1 +  {\dashint_{-1}^1   \frac{ P_a\left(u_2 \right) }{u_2-\tau_2(x)} \d u_2},
\end{align*}
%
where $P_f(u_1) = p_f(x(u_1))$ and $P_a(u_2) = p_a(x(u_1))$. 

We now consider $\tau_1$ and $\tau_2$ as independent variables and seek an expansion of the pressure distribution in terms of Jacobi polynomials: 
%
\begin{align*}
P_f(\tau_1) &= p_0^- \frac{(1-\tau_1)^{\gamma}}{(1+\tau_1)^{1/2} }+ (1-\tau_1)^{\gamma}( 1+\tau_1 )^{1/2}\sum_{n=1}^\infty p_n^- P_{n-1}^{\gamma,1/2} \left( \tau_1 \right),  \\
P_a(\tau_2) &= (1-\tau_2)^\gamma(1+\tau_2)^\alpha \sum_{n=1}^\infty p_n^+ P_{n-1}^{\alpha,\gamma} \left( \tau_2\right).
\end{align*}
%
\iffalse
so that
%
\begin{align*}
I_f(\tau_1) &= p_0^- w^{\gamma,-1/2}(\tau_1) Q_0^{\gamma,-1/2}(\tau_1) + \weight{\tau_1}{\gamma}{1/2} \sum_{n=1}^\infty p_n^- Q_{n-1}^{\gamma,1/2} (  \tau_1 ), \\
I_a(\tau_2)&=\weight{\tau_2}{\alpha}{\gamma} \sum_{n=1}^\infty p_n^+ Q_{n-1}^{\alpha,\gamma} ( \tau_2 ).
\end{align*}
%
However, we must note a subtlety in the interpretation of $Q$. When $\tau_1 \neq [-1,1]$ then we must use the alternative representation for $Q$.
\fi
Substitution of these representations into \eqref{Eq:ppGE} yields equations on the forward and aft parts of the aerofoils. On $-1<x<c$ we have
%
\begin{align}
- \left(p_0^- w^{\gamma,-1/2}(\tau_1) Q_0^{\gamma,-1/2}(\tau_1) + \weight{\tau_1}{\gamma}{1/2} \sum_{n=1}^\infty p_n^- Q_{n-1}^{\gamma,1/2} (  \tau_1 ) \right. \notag \\
\left.+\weight{\tau_2}{\alpha}{\gamma} \sum_{n=1}^\infty p_n^+ Q_{n-1}^{\alpha,\gamma} ( \tau_2 ) \right)  = 4 \pi \frac{\d z}{\d x}(x(\tau_1)),
\label{Eq:ppColFor}
\end{align}
%
and on $c<x<1$ we have
%
\begin{align}
\pi \psi_0 w^{\gamma, \alpha}(\tau_2) \sum_{n=1}^\infty p_n^+ P_{n-1}^{\alpha,\gamma} \left( \tau_2\right)- \left( p_0^- w^{\gamma,-1/2}(\tau_1) Q_0^{\gamma,-1/2}(\tau_1) + \weight{\tau_1}{\gamma}{1/2} \sum_{n=1}^\infty p_n^- Q_{n-1}^{\gamma,1/2} (  \tau_1 ) \right. \notag \\
\left.+\weight{\tau_2}{\alpha}{\gamma} \sum_{n=1}^\infty p_n^+ Q_{n-1}^{\alpha,\gamma} ( \tau_2 )\right)  = 4\pi \frac{\d z}{\d x}(x(\tau_2)). \label{Eq:ppColAft}
\end{align}
%
\iffalse
We now truncate the series at $N-$ and $N^-$ to obtain, for $-1<x<c$,
%
\begin{align}
\frac{1+c}{2} \left( p_0^- w^{\gamma,-1/2}(\tau_1) Q_0^{\gamma,-1/2}(\tau_1) + \weight{\tau_1}{\gamma}{1/2} \sum_{n=1}^{N^-} p_n^- Q_{n-1}^{\gamma,1/2} (  \tau_1 ) \right) \notag \\
+\frac{1-c}{2} \weight{\tau_2}{\alpha}{\gamma} \sum_{n=1}^{N^+} p_n^+ Q_{n-1}^{\alpha,\gamma} ( \tau_2 )  = 4 \pi \frac{\d z}{\d x}(x(\tau_1)). \label{Eq:ppJacExp1}
\end{align}
%
and for $c<x<1$,
%
\begin{align}
\frac{1+c}{2} \left( p_0^- w^{\gamma,-1/2}(\tau_1) Q_0^{\gamma,-1/2}(\tau_1) + \weight{\tau_1}{\gamma}{1/2} \sum_{n=1}^{N^-} p_n^- Q_{n-1}^{\gamma,1/2} (  \tau_1 ) \right) \notag \\
+\sum_{n=1}^{N^+} p_n^+ \left( 2 \pi \psi(x)w^{\alpha,\gamma}(\tau_2)  P_{n-1}^{\alpha,\gamma} \left( \tau_2\right) +  \frac{1-c}{2} \weight{\tau_2}{\alpha}{\gamma} Q_{n-1}^{\alpha,\gamma} ( \tau_2 )  \right) = 4 \pi \frac{\d z}{\d x}(x(\tau_2)).
\label{Eq:ppJacExp2}
\end{align}
\fi
%\subsection{Constructing the linear system}
Similarly to the case for continuous porosity distributions, we truncate \eqref{Eq:ppColFor} and \eqref{Eq:ppColAft} at $N_-$ and $N_+$ respectively. We consider \eqref{Eq:ppColFor} as a function of $\tau_1$ and collocate at the zeros of $P_{N_-+1}^{\gamma, 1/2}$. Conversely, we consider \eqref{Eq:ppColAft} as a function of $\tau_2$ and collocate at the zeros of $P_{N^+}^{\alpha,\gamma}$. This generates a linear $(N_-+N_++1)\times (N_-+N_++1)$ system. By using similar reasoning to the previous section, we may show that the rows of the associated matrix are linearly independent, and the matrix is therefore invertible and the system is considered solved.

\iffalse
We now construct a linear system of equations. We do this via Jacobi collocation.

First consider \eqref{Eq:ppJacExp1}. We consider the Jacobi nodes (i.e. the roots) of the $N^-$-th Jacobi polynomial. This provides $N^-$ polynomials for $N^-+1$ unknowns. Secondly, do a similar thing with \eqref{Eq:ppJacExp2}. Consider the Jacobi nodes for the $N^+$-th Jacobi polynomial. Then we have $N^+$ equations for $N^+$ unknowns. Finally, we apply the system by using \eqref{Eq:ppPJump}.
%
Consider the vector 
%
\begin{align*}
\mathbf{p}&=
  \begin{bmatrix}
p_0^-\\
p_1^- \\
\vdots \\
p_{N^-}^-\\
p_1^+ \\
\vdots\\
p_{N^+}^+
\end{bmatrix}
\end{align*}
%
So that
%
\begin{align*}
\mathbf{A} \mathbf{p} &= \mathbf{z}
\end{align*}

So that 

\begin{align*}
 \mathbf{p} &= \mathbf{A}^{-1} \mathbf{z}
\end{align*}
\fi
\iffalse
\subsection{Expressions for aerodynamic quantities}
%
Similarly to the case for continuous porosity distributions, compact expressions are now available for key aerodynamic quantities. For example, the lift may be expressed as 
%
\begin{align*}
c_L & = \int_{-1}^1 p(t) \d t.
\end{align*}
%
We now derive expressions for important aerodynamic quantities. The lift is given by [need to complete].
%

\fi

==> sections/partially-porous.tex <==
\subsection{Solution for discontinuous porosity distributions}

We may also use the expansion for a partially porous aerofoil. A practical application of interest is  an aerofoil with a in impermeable forward section and a permeable aft section. If we place the permeable-impermeable junction at $x = a$, then we would write the singular integral equation for a steady, partially porous aerofoil as 

\begin{align}
H(x - c) \psi(x) p(x)-\frac{1}{2\pi}\dashint_{-1}^{1}\frac{p(t)}{t-x}dt~=~2\frac{dz}{dx} \label{Eq:ppGE}
\end{align}

where $H(\cdot)$ is the heaviside function, i.e.

\begin{align}
    H(x - c) = \begin{cases}
    0 & x<c \\
    1 & x>c
    \end{cases}
\end{align}

We first note that we require $p=0$ at $x = c$. Otherwise there would be a discontinuity in the seepage velocity.

Therefore, we seek an expansion of the form

\begin{align}
    p(x) & = \frac{(1-x)^\alpha}{(1+x)^\beta} |c-x|^\gamma \tilde{p}(x) \label{Eq:ppFact}
\end{align}

We apply similar arguments to the previous sections to yield

\begin{align*}
    \alpha &= \frac{1}{\pi} \cot^{-1}(\psi(-1)) \\
    \beta &= \frac{1}{\pi} \cot^{-1}(\psi(\phantom{-}1))
\end{align*}

We may write the pressure in the form 

\begin{align}
p(x) &= p^\ast(x) (x-c)^\gamma, && p^\ast = \frac{(1-x)^\alpha}{(1+x)^\beta} \e^{\i \pi \gamma H(c-x)} \tilde{p}(x) \label{Eq:pDiscFac}
\end{align}

so that 

\begin{align*}
p^\ast(c^-) &= \frac{(1-c)^\alpha}{(1+c)^\beta} \e^{\i \pi \gamma} \tilde{p}(c^-)\\
p^\ast(c^+) &= \frac{(1-c)^\alpha}{(1+c)^\beta} \tilde{p}(c^+)
\end{align*}

and apply the results of \eqref{Eq:plemeljDiscLim}.

If we substitute \eqref{Eq:pDiscFac} into \eqref{Eq:ppGE} and consider the limit $x \rightarrow a^-$ then we obtain (at leading order)

\begin{align*}
0 - \i \left(-\frac{\e^{-\i \gamma \pi} }{2 \i \sin(\gamma \pi)} \frac{(1-c)^\alpha}{(1+c)^\beta} \tilde{p}(c^+) + \frac{\cot(\gamma \pi)}{2 \i } \frac{(1-c)^\alpha}{(1+c)^\beta} \e^{\i \pi \gamma} \tilde{p}(c^-)\right) \cdot \left(t_0 - c\right)^\gamma + \Phi_0^\ast(t_0) &= ~2\frac{dz}{dx}
\end{align*}
Since every power of zero must vanish, we require

\begin{align}
\tilde{p}(c^+) =\cos(\gamma \pi)\e^{2 \i \pi \gamma} \tilde{p}(c^-) \label{Eq:ppPJump}
\end{align}

If we now consider $x \rightarrow a^+$ then we obtain

\begin{align*}
\psi(c^+)  \frac{(1-c)^\alpha}{(1+c)^\beta} \tilde{p}(c^+) (x-c)^\gamma +  \i \left(\frac{\e^{\i \gamma \pi}}{2 \i \sin(\gamma \pi)} \frac{(1-c)^\alpha}{(1+c)^\beta} \e^{\i \pi \gamma} \tilde{p}(c^-) - \frac{\cot(\gamma \pi)}{2 \i } \frac{(1-c)^\alpha}{(1+c)^\beta} \tilde{p}(c^+) \right) \cdot \left(t_0 - c\right)^\gamma + \Phi_0^\ast(t_0) &= ~2\frac{dz}{dx}
\end{align*}

To get 

\begin{align*}
\psi(c^+) \tilde{p}(c^+) - \i \left(\frac{\e^{\i \gamma \pi}}{2 \i \sin(\gamma \pi)} \e^{\i \pi \gamma} \tilde{p}(c^-) - \frac{\cot(\gamma \pi)}{2 \i } \tilde{p}(c^+) \right)&=0
\end{align*}

Using \eqref{Eq:ppPJump} we obtain

\begin{align*}
\psi(c^+) \cos(\gamma \pi)\e^{2 \i \pi \gamma} \tilde{p}(c^-)+ \i \left(\frac{\e^{\i \gamma \pi}}{2 \i \sin(\gamma \pi)} \e^{\i \pi \gamma} \tilde{p}(c^-) - \frac{\cot(\gamma \pi)}{2 \i } \ \cos(\gamma \pi)\e^{2 \i \pi \gamma} \tilde{p}(c^-) \right)&=0
\end{align*}

Rearranging gives

\begin{align*}
\psi(c^+) \cos(\gamma \pi)+ \left(\frac{1}{2 \i \sin(\gamma \pi)}  - \frac{\cot(\gamma \pi)}{2 \i }  \cos(\gamma \pi) \right)&=0
\end{align*}
%
which has the solution
%
\begin{align*}
\gamma &= \frac{\arctan(2 \psi(c^+))}{\pi} = \frac{1}{2} - \frac{\arccos(2 \psi(c^+))}{\pi} 
\end{align*}
%
We define $\kappa = \frac{\arccos(2 \psi(c^+))}{\pi}$.
%
Therefore we may express \eqref{Eq:ppFact} as 
%
\begin{align}
p(x) & = \frac{(1-x)^\alpha}{(1+x)^\beta} \frac{|c-x|^{1/2}}{|c-x|^{\arccos(2 \psi(c^+))/\pi}} \tilde{p}(x) 
\end{align}
%
When the wing is partially porous, we may write
%
\begin{align}
p(x) & = \left|\frac{ x-c }{ x +1} \right|^{1/2} \cdot \left| \frac{x-1}{x-c} \right|^{\kappa} \tilde{p}(x) 
\end{align}

which is equivalent to \cite[eq. (13)]{gil2}. Consequently, we seek solutions of the form

\begin{align*}
p(x) &= \begin{dcases}
p_0^- \frac{(c-x)^{\gamma}}{(1+x)^{1/2} }+ \left(  \frac{4 (x-c)(x+1)}{(c+1)^2} \right)^\gamma \sum_{n=1}^\infty p_n^- P_{n-1}^{\gamma,\gamma} \left( \frac{2 (1+x)}{1+c} -1  \right) & -1 < x \leq c \\
\sqrt{\frac{2}{1-c} } (x-c)^\gamma(1-x)^\beta\sum_{n=1}^\infty p_n^+ P_{n-1}^{\beta,\gamma} \left( 1+  \frac{2 (x-1)}{1-c} \right)  & c<x<1
\end{dcases}
\end{align*}

We normalise  the domain by using
\begin{align*}
\tau_1(x) &= -1+2 \frac{x+1}{1+c}, & -1<x<c\\
\tau_2(x) &= \phantom{-} 1+ 2 \frac{x-1}{1-c}, &c<x<1
\end{align*}
%
and the equivalent inversions
%
\begin{align*}
x(\tau_1) &= -1+ \frac{(\tau_1+1)(1+c)}{2}, & -1<x<c\\
x(\tau_2) &= \phantom{-} 1+ \frac{(\tau_2-1)(1-c)}{2}, &c<x<1
\end{align*}
%
Note that
%
\begin{align*}
\tau_1 = \phantom{-}1+ (\tau_2+1)\frac{1-c}{1+c}\\
\tau_2 = -1+ (\tau_1-1)\frac{1+c}{1-c}
\end{align*}
%
We split the integral appropriately
%
\begin{align*}
\dashint_{-1}^1 \frac{p(t)}{t-x} \d t &= \dashint_{-1}^c  \frac{p_f(t) }{t-x} \d t + \dashint_{c}^1 \frac{ p_a(t)  }{t-x} \d t\\
& = \frac{1+c}{2}  \dashint_{-1}^1   \frac{p_f\left(t(u_1) \right) }{t(u_1)-x} \d u_1 +  \frac{1-c}{2}  \dashint_{-1}^1   \frac{ p_a\left(t(u_2) \right) }{t(u_2)-x} \d u_2 \\
& = \underbrace{\dashint_{-1}^1   \frac{P_f\left(u_1\right) }{u_1-\tau_1(x)} \d u_1}_{\coloneqq I_f(\tau_1)} +  \underbrace{\dashint_{-1}^1   \frac{ P_a\left(u_2 \right) }{u_2-\tau_2(x)} \d u_2}_{\coloneqq I_a(\tau_2)} \\
\end{align*}
%
where $P_f(u_1) = p_f(t(u_1))$ and $P_a(u_2) = p_a(t(u_1))$. We now consider $\tau_1$ and $\tau_2$ as the independent variables and write 
%
\begin{align*}
P_f(\tau_1) &= p_0^- \frac{(1-\tau_1)^{\gamma}}{(1+\tau)^{1/2} }+ \left( 1-\tau_1^2 \right)^\gamma \sum_{n=1}^\infty p_n^- P_{n-1}^{\gamma,\gamma} \left( \tau_1 \right)  \\
P_a(\tau_2) &= (\tau_2-1)^\gamma(1+\tau_2)^\beta \sum_{n=1}^\infty p_n^+ P_{n-1}^{\beta,\gamma} \left( \tau_2\right)
\end{align*}
%
so that
%
\begin{align*}
I_f(\tau_1) &=\left( p_0^- w^{\gamma,-1/2}(\tau_1) Q_0^{\gamma,-1/2}(\tau_1) + \weight{\tau_1}{\gamma}{\gamma} \sum_{n=1}^\infty p_n^- Q_{n-1}^{\gamma,\gamma} (  \tau_1 ) \right) \\
I_a(\tau_2)&=\weight{\tau_2}{\beta}{\gamma} \sum_{n=1}^\infty p_n^+ Q_{n-1}^{\beta,\gamma} ( \tau_2 )
\end{align*}
%
However, we must note a subtlety in the interpretation of $Q$. When $\tau_1 \neq [-1,1]$ then we must use the alternative representation for $Q$.
Therefore we have, for $-1<x<c$,

\begin{align*}
\left( p_0^- w^{\gamma,-1/2}(\tau_1) Q_0^{\gamma,-1/2}(\tau_1) + \weight{\tau_1}{\gamma}{\gamma} \sum_{n=1}^\infty p_n^- Q_{n-1}^{\gamma,\gamma} (  \tau_1 ) \right) \\
+\weight{\tau_2}{\beta}{\gamma} \sum_{n=1}^\infty p_n^+ Q_{n-1}^{\beta,\gamma} ( \tau_2 )  = 4 \pi \frac{\d z}{\d x}(x(\tau_1))
\end{align*}

and for $c<x<1$,

\begin{align*}
\psi_0 w^{\gamma, \beta}(\tau_2) \sum_{n=1}^\infty p_n^+ P_{n-1}^{\beta,\gamma} \left( \tau_2\right)+ \left( p_0^- w^{\gamma,-1/2}(\tau_1) Q_0^{\gamma,-1/2}(\tau_1) + \weight{\tau_1}{\gamma}{\gamma} \sum_{n=1}^\infty p_n^- Q_{n-1}^{\gamma,\gamma} (  \tau_1 ) \right) \\
+\weight{\tau_2}{\beta}{\gamma} \sum_{n=1}^\infty p_n^+ Q_{n-1}^{\beta,\gamma} ( \tau_2 )  = 4 \pi \frac{\d z}{\d x}(x(\tau_2))
\end{align*}
%
We now truncate the series at $N-$ and $N^-$ to obtain, for $-1<x<c$,
%
\begin{align}
\frac{1+c}{2} \left( p_0^- w^{\gamma,-1/2}(\tau_1) Q_0^{\gamma,-1/2}(\tau_1) + \weight{\tau_1}{\gamma}{\gamma} \sum_{n=1}^{N^-} p_n^- Q_{n-1}^{\gamma,\gamma} (  \tau_1 ) \right) \\
+\frac{1-c}{2} \weight{\tau_2}{\beta}{\gamma} \sum_{n=1}^{N^+} p_n^+ Q_{n-1}^{\beta,\gamma} ( \tau_2 )  = -4 \pi \frac{\d z}{\d x}(x(\tau_1)) \label{Eq:ppJacExp1}
\end{align}
%
and for $c<x<1$,
%
\begin{align}
\frac{1+c}{2} \left( p_0^- w^{\gamma,-1/2}(\tau_1) Q_0^{\gamma,-1/2}(\tau_1) + \weight{\tau_1}{\gamma}{\gamma} \sum_{n=1}^{N^-} p_n^- Q_{n-1}^{\gamma,\gamma} (  \tau_1 ) \right) \\
+\sum_{n=1}^{N^+} p_n^+ \left( 2 \pi \psi(x)(\tau_2-1)^\gamma(1+\tau_2)^\beta  P_{n-1}^{\beta,\gamma} \left( \tau_2\right) +  \frac{1-c}{2} \weight{\tau_2}{\beta}{\gamma} Q_{n-1}^{\beta,\gamma} ( \tau_2 )  \right) = 4 \pi \frac{\d z}{\d x}(x(\tau_2))
\label{Eq:ppJacExp2}
\end{align}
\subsection{Constructing the linear system}

We now construct a linear system of equations. We do this via Jacobi collocation.

First consider \eqref{Eq:ppJacExp1}. We consider the Jacobi nodes (i.e. the roots) of the $N^-$-th Jacobi polynomial. This provides $N^-$ polynomials for $N^-+1$ unknowns. Secondly, do a similar thing with \eqref{Eq:ppJacExp2}. Consider the Jacobi nodes for the $N^+$-th Jacobi polynomial. Then we have $N^+$ equations for $N^+$ unknowns. Finally, we apply the system by using \eqref{Eq:ppPJump}.
%
Consider the vector 
%
\begin{align*}
\mathbf{p}&=
  \begin{bmatrix}
p_0^-\\
p_1^- \\
\vdots \\
p_{N^-}^-\\
p_1^+ \\
\vdots\\
p_{N^+}^+
\end{bmatrix}
\end{align*}
%
So that
%
\begin{align*}
\mathbf{A} \mathbf{p} &= \mathbf{z}
\end{align*}

So that 

\begin{align*}
 \mathbf{p} &= \mathbf{A}^{-1} \mathbf{z}
\end{align*}


==> sections/pp-aoa-val.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{tikzpicture}[%
trim axis left, trim axis right
]

\begin{axis}[%
width=0.951\fwidth,
height=\fheight,
at={(0\fwidth,0\fheight)},
scale only axis,
xmin=0,
xmax=40,
xlabel style={font=\color{white!15!black}},
xlabel={$n$},
ymode=log,
ymin=7.25899823149149e-16,
ymax=1,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={$\epsilon_n$},
axis background/.style={fill=white}
]
\addplot [color=mycolor1, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
1	0.156201812258151\\
2	0.0208882932604403\\
3	0.0213499980408695\\
4	0.00308555325275789\\
5	0.00317445482200017\\
6	0.000486196712587722\\
7	0.000492227163865991\\
8	7.56521266904218e-05\\
9	7.69082102255414e-05\\
10	1.21707156815053e-05\\
11	1.22765555031371e-05\\
12	1.9453734923106e-06\\
13	1.96800262815591e-06\\
14	3.17522450918225e-07\\
15	3.19646771173952e-07\\
16	5.15466258780695e-08\\
17	5.20009125629011e-08\\
18	8.48460240257872e-09\\
19	8.53068673544315e-09\\
20	1.39118946713987e-09\\
21	1.40100640684651e-09\\
22	2.30373519511491e-10\\
23	2.31425225261029e-10\\
24	3.80357372576508e-11\\
25	3.82583008180007e-11\\
26	6.32681995183112e-12\\
27	6.35245594082575e-12\\
28	1.0502031256483e-12\\
29	1.05461239281295e-12\\
30	1.75246020773029e-13\\
31	1.75765607063285e-13\\
32	2.990093549961e-14\\
33	3.01411031277384e-14\\
34	7.9162213924998e-15\\
35	7.79805421639909e-15\\
36	6.22179211896666e-15\\
37	6.85057728633269e-15\\
38	6.30947734951087e-15\\
40	6.07056058387665e-15\\
};
\addplot [color=mycolor2, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
1	0.126918929000956\\
2	0.0165072813631303\\
3	0.0167916366188068\\
4	0.00241210531809245\\
5	0.00245881250470631\\
6	0.000371303916012205\\
7	0.000374829799410814\\
8	5.75850132210156e-05\\
9	5.82177810481251e-05\\
10	9.16244593578972e-06\\
11	9.22133324616961e-06\\
12	1.46167170658136e-06\\
13	1.47274280802792e-06\\
14	2.36722199420435e-07\\
15	2.37863993780329e-07\\
16	3.83776917577328e-08\\
17	3.85951575288647e-08\\
18	6.28281626790008e-09\\
19	6.30694955899904e-09\\
20	1.02914511428831e-09\\
21	1.03376520242671e-09\\
22	1.69732764074883e-10\\
23	1.70272316695428e-10\\
24	2.80024935877515e-11\\
25	2.81061075320262e-11\\
26	4.64344172822994e-12\\
27	4.65590996069148e-12\\
28	7.70288912507758e-13\\
29	7.72438709782966e-13\\
30	1.28238368358895e-13\\
31	1.28618240660402e-13\\
32	2.13577889352533e-14\\
33	2.12989393431856e-14\\
34	4.97440067912661e-15\\
35	4.60164619759076e-15\\
36	3.400835459158e-15\\
38	3.20222859859506e-15\\
39	3.20896323659881e-15\\
40	3.34626161649102e-15\\
};
\addplot [color=mycolor3, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
1	0.105031387884895\\
2	0.0135579113093644\\
3	0.0137255354956483\\
4	0.00196970899198258\\
5	0.00199284287100435\\
6	0.000299268865766942\\
7	0.000301346270835946\\
8	4.64106687381156e-05\\
9	4.67262156298797e-05\\
10	7.34037226797691e-06\\
11	7.37397979054263e-06\\
12	1.17156922939419e-06\\
13	1.17695680323814e-06\\
14	1.89032124921547e-07\\
15	1.89666570555788e-07\\
16	3.06595829701684e-08\\
17	3.07643216475025e-08\\
18	5.00704341263537e-09\\
19	5.02017068019492e-09\\
20	8.20470870437427e-10\\
21	8.22676283366404e-10\\
22	1.35083391498526e-10\\
23	1.35371857812401e-10\\
24	2.22927094465665e-11\\
25	2.23418100590358e-11\\
26	3.69162261172622e-12\\
27	3.6983175308264e-12\\
28	6.12355315718981e-13\\
29	6.13440974308476e-13\\
30	1.01872239420955e-13\\
31	1.0194607425442e-13\\
32	1.69353459011125e-14\\
33	1.69208760383259e-14\\
34	3.0963524308005e-15\\
35	3.16226356320028e-15\\
36	1.36642954865414e-15\\
37	1.49463110030536e-15\\
38	1.43715600521107e-15\\
39	1.44485381637983e-15\\
40	1.59817449738279e-15\\
};
\addplot [color=mycolor4, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
1	0.0891393043745912\\
2	0.0114605280979403\\
3	0.0115293730636559\\
4	0.00164910358520793\\
5	0.00165771198207001\\
6	0.000248507198368895\\
7	0.000249415922883325\\
8	3.84553701539475e-05\\
9	3.85774493850991e-05\\
10	6.05857902286882e-06\\
11	6.07329178889152e-06\\
12	9.66184835047084e-07\\
13	9.68293480454937e-07\\
14	1.55555858973045e-07\\
15	1.55831240188106e-07\\
16	2.52198455433257e-08\\
17	2.52609613577552e-08\\
18	4.11302029027604e-09\\
19	4.11866678636363e-09\\
20	6.73822754133134e-10\\
21	6.74688619151946e-10\\
22	1.10833975922069e-10\\
23	1.10956985284386e-10\\
24	1.82884879223872e-11\\
25	1.8307629285395e-11\\
26	3.02648489415767e-12\\
27	3.02927903391446e-12\\
28	5.02000959157589e-13\\
29	5.02432620732297e-13\\
30	8.34435559933184e-14\\
31	8.35504978030896e-14\\
32	1.38673391381177e-14\\
33	1.38585858637078e-14\\
34	2.39644443420633e-15\\
35	2.43007197882934e-15\\
36	7.25899823149152e-16\\
37	9.3003449000733e-16\\
38	9.27364669398794e-16\\
39	1.05751602226074e-15\\
40	8.6014883588854e-16\\
};
\end{axis}
\end{tikzpicture}%

==> sections/pp-cam-val.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{tikzpicture}[%
trim axis left, trim axis right
]

\begin{axis}[%
width=0.951\fwidth,
height=\fheight,
at={(0\fwidth,0\fheight)},
scale only axis,
xmin=0,
xmax=40,
xlabel style={font=\color{white!15!black}},
xlabel={$n$},
ymode=log,
ymin=5.59950137558246e-16,
ymax=1,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={$\epsilon_n$},
axis background/.style={fill=white}
]
\addplot [color=mycolor1, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
1	0.339553430233659\\
2	0.017090100740359\\
3	0.0145359528291223\\
4	0.00137307583962665\\
5	0.00140564787261953\\
6	0.000187657940713997\\
7	0.000162324000446179\\
8	2.07125173579295e-05\\
9	2.09055735053325e-05\\
10	3.06029241665578e-06\\
11	2.57938529796931e-06\\
12	4.19829102081856e-07\\
13	3.71697402155933e-07\\
14	6.54744140241005e-08\\
15	5.58276005676486e-08\\
16	9.52905874502466e-09\\
17	8.44840897817639e-09\\
18	1.52754756318375e-09\\
19	1.31618500154488e-09\\
20	2.30401628274171e-10\\
21	2.05028210532306e-10\\
22	3.75382385474613e-11\\
23	3.26495388830245e-11\\
24	5.7982741311256e-12\\
25	5.18239566575309e-12\\
26	9.551266694756e-13\\
27	8.37200553656596e-13\\
28	1.49751979626331e-13\\
29	1.34531881669246e-13\\
30	2.58228452741315e-14\\
31	2.2785648411641e-14\\
32	6.54643087927347e-15\\
33	6.59788125715195e-15\\
34	5.60127626769036e-15\\
35	5.37451956587723e-15\\
36	5.39068302410495e-15\\
38	5.84844247995854e-15\\
39	5.30861386348285e-15\\
40	5.59182810841158e-15\\
};
\addplot [color=mycolor2, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
1	0.189867814310305\\
2	0.0107697081622152\\
3	0.00979527017746435\\
4	0.00109886290771463\\
5	0.00101691442063038\\
6	0.000137978067996227\\
7	0.000126548881970318\\
8	1.86939608401573e-05\\
9	1.71534496184986e-05\\
10	2.68416548071787e-06\\
11	2.48411323471711e-06\\
12	4.00859016456011e-07\\
13	3.72205541328966e-07\\
14	6.10592117278889e-08\\
15	5.70885418091433e-08\\
16	9.49647029659133e-09\\
17	8.90289125281994e-09\\
18	1.49243807715633e-09\\
19	1.40678408158308e-09\\
20	2.3755961364747e-10\\
21	2.24421239978708e-10\\
22	3.80511339469817e-11\\
23	3.61019486544808e-11\\
24	6.14712063388647e-12\\
25	5.84293661753916e-12\\
26	9.96940526377794e-13\\
27	9.51060431558285e-13\\
28	1.62695892878682e-13\\
29	1.55736429187956e-13\\
30	2.68045391532068e-14\\
31	2.54757163603744e-14\\
32	5.0036072828765e-15\\
33	5.1774099237984e-15\\
34	2.39168388675492e-15\\
35	2.68655781792022e-15\\
36	2.32794804512281e-15\\
37	2.46804385322059e-15\\
39	2.19982214709647e-15\\
40	2.19027081223214e-15\\
};
\addplot [color=mycolor3, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
1	0.158754954099513\\
2	0.00945157839501553\\
3	0.00906115513972334\\
4	0.00103271493245994\\
5	0.000980309525370978\\
6	0.000131651764846857\\
7	0.000126689769981056\\
8	1.85354095655726e-05\\
9	1.78114934034314e-05\\
10	2.7106677429936e-06\\
11	2.62612629622414e-06\\
12	4.12320544631574e-07\\
13	3.99245513073632e-07\\
14	6.36008708251179e-08\\
15	6.1939072541017e-08\\
16	1.00216791768975e-08\\
17	9.75674589636343e-09\\
18	1.58940565129902e-09\\
19	1.55392366259779e-09\\
20	2.55478218688243e-10\\
21	2.49715943157136e-10\\
22	4.12037868139997e-11\\
23	4.04038466115487e-11\\
24	6.70724045778976e-12\\
25	6.57564735342241e-12\\
26	1.09396410437198e-12\\
27	1.07506566764972e-12\\
28	1.79601715373844e-13\\
29	1.7648921909398e-13\\
30	2.94747437217119e-14\\
31	2.90175299089403e-14\\
32	4.97255947846402e-15\\
33	4.97633530922861e-15\\
34	1.20679148556243e-15\\
35	1.31360581182313e-15\\
36	1.11109960402039e-15\\
37	1.16251802823663e-15\\
38	1.02267650760022e-15\\
39	8.2941179046415e-16\\
40	8.93300842969525e-16\\
};
\addplot [color=mycolor4, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
1	0.14714039074789\\
2	0.00891246383857316\\
3	0.00879824802974367\\
4	0.000992948351837807\\
5	0.000976305279407831\\
6	0.000130151311474017\\
7	0.000128550337606193\\
8	1.85519270015656e-05\\
9	1.83256129553843e-05\\
10	2.756898398817e-06\\
11	2.72964710186381e-06\\
12	4.22318915186868e-07\\
13	4.18203341391521e-07\\
14	6.5832610145632e-08\\
15	6.52981943186509e-08\\
16	1.04219319145122e-08\\
17	1.03385128572014e-08\\
18	1.66520713230043e-09\\
19	1.65385072789265e-09\\
20	2.68546897746361e-10\\
21	2.66735358969096e-10\\
22	4.35510242700158e-11\\
23	4.32963385990506e-11\\
24	7.10655556461338e-12\\
25	7.06536302228488e-12\\
26	1.16391081834591e-12\\
27	1.15799951842783e-12\\
28	1.91531756921027e-13\\
29	1.90553940716506e-13\\
30	3.15463630519473e-14\\
31	3.14413628301608e-14\\
32	5.25362035679425e-15\\
33	5.23189999480268e-15\\
34	1.03706851040411e-15\\
35	1.04968122240583e-15\\
36	6.13397941947437e-16\\
37	7.16389875351832e-16\\
38	5.9051771500648e-16\\
39	5.59950137558242e-16\\
40	5.65301931602641e-16\\
};
\end{axis}
\end{tikzpicture}%

==> sections/pp-press-aoa.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{tikzpicture}[%
trim axis left, trim axis right
]

\begin{axis}[%
width=0.951\fwidth,
height=\fheight,
at={(0\fwidth,0\fheight)},
scale only axis,
unbounded coords=jump,
xmin=-1,
xmax=1,
xlabel style={font=\color{white!15!black}},
xlabel={$x$},
ymin=0,
ymax=12,
ylabel style={font=\color{white!15!black}},
ylabel={$\left|p / \alpha \right|$},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left
]
\addplot[only marks, mark=+, mark options={}, mark size=1.5000pt, draw=mycolor1] table[row sep=crcr]{%
x	y\\
-1	inf\\
-0.963458378673011	27.314427792587\\
-0.859174675048864	13.4585289293576\\
-0.702391671561197	8.75938701920063\\
-0.516025788785828	6.35882310708118\\
-0.327317472789346	4.88704719612416\\
-0.163849554869341	3.88110919038644\\
-0.0495155660487905	3.09916800969595\\
-0.00102730362483183	2.01355397290478\\
0.0163525684804853	2.48401669140495\\
0.0992931890660217	2.76658622610123\\
0.240803715844737	2.65702739805698\\
0.42020005248331	2.3522032209917\\
0.611260466978157	1.95383646853517\\
0.786058330061085	1.50763076019082\\
0.91904405244592	1.01188300490687\\
0.990779578495533	0.423162107901038\\
};
\addplot [color=mycolor1, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
-1	inf\\
-0.998972696375168	164.622308605041\\
-0.995895006911623	82.2773335098419\\
-0.990779578495533	54.8140105870297\\
-0.983647431519515	41.0711386185257\\
-0.974527873505334	32.8164897181359\\
-0.963458378673011	27.3059984060254\\
-0.95048443395121	23.363645802439\\
-0.935659352061695	20.401430707695\\
-0.91904405244592	18.0926933192056\\
-0.900706810933978	16.2414447344053\\
-0.880722979184567	14.7229712787372\\
-0.859174675048864	13.454136670076\\
-0.836150445130658	12.3773908681708\\
-0.811744900929367	11.4516322562332\\
-0.786058330061085	10.6467249206625\\
-0.759196284155263	9.94007190876972\\
-0.731269145120418	9.31439786777868\\
-0.702391671561197	8.75627072920147\\
-0.672682527210654	8.25509013362495\\
-0.642263793315516	7.80237920668682\\
-0.611260466978157	7.39127853303761\\
-0.57979994751669	7.01617794902598\\
-0.548011512953841	6.67244415665885\\
-0.516025788785828	6.35621614712413\\
-0.483974211214172	6.06424936938044\\
-0.451988487046159	5.79379542474277\\
-0.42020005248331	5.54250795925708\\
-0.388739533021843	5.30836805782996\\
-0.357736206684484	5.08962424849973\\
-0.327317472789346	4.88474347335683\\
-0.297608328438803	4.69237024730936\\
-0.268730854879582	4.51129181703574\\
-0.240803715844737	4.34040751762777\\
-0.213941669938915	4.1787007399212\\
-0.188255099070633	4.02521197636673\\
-0.163849554869341	3.87901128609096\\
-0.140825324951136	3.73916814545449\\
-0.119277020815433	3.60471588865315\\
-0.0992931890660217	3.4746065079991\\
-0.0809559475540796	3.34764888460515\\
-0.0643406479383053	3.22241827860602\\
-0.0495155660487905	3.09711417166305\\
-0.0365416213269891	2.96931992020832\\
-0.0254721264946658	2.83556053347369\\
-0.0163525684804853	2.69039850798445\\
-0.00922042150446734	2.5242999430947\\
-0.00410499308837697	2.31737387991492\\
-0.00102730362483183	2.01201601621391\\
0	0\\
0	0\\
0.00102730362483183	1.91000579379389\\
0.00410499308837692	2.18772847004151\\
0.00922042150446734	2.36123492395952\\
0.0163525684804853	2.48449716154988\\
0.0254721264946657	2.57589771093037\\
0.0365416213269891	2.64414281561147\\
0.0495155660487904	2.69416415127248\\
0.0643406479383053	2.7291137703001\\
0.0809559475540797	2.75119723763418\\
0.0992931890660217	2.7620712216727\\
0.119277020815433	2.76305119952759\\
0.140825324951136	2.75522711167137\\
0.163849554869342	2.73953082324174\\
0.188255099070633	2.71677690119671\\
0.213941669938915	2.68768801750209\\
0.240803715844737	2.65291125427462\\
0.268730854879582	2.61302893638439\\
0.297608328438803	2.56856614557599\\
0.327317472789346	2.51999621754298\\
0.357736206684484	2.46774501279621\\
0.388739533021843	2.41219443919458\\
0.42020005248331	2.3536855094891\\
0.451988487046159	2.29252109575748\\
0.483974211214172	2.22896846704704\\
0.516025788785828	2.16326165010866\\
0.548011512953841	2.09560362508962\\
0.57979994751669	2.0261683514649\\
0.611260466978157	1.95510260964953\\
0.642263793315516	1.88252763743591\\
0.672682527210654	1.80854053532106\\
0.702391671561197	1.73321540910564\\
0.731269145120418	1.656604210184\\
0.759196284155263	1.57873722184869\\
0.786058330061085	1.49962312124084\\
0.811744900929367	1.4192485175967\\
0.836150445130659	1.33757682218585\\
0.859174675048864	1.25454623361262\\
0.880722979184567	1.17006650584045\\
0.900706810933978	1.08401397183778\\
0.91904405244592	0.996223957990336\\
0.935659352061695	0.906479109945087\\
0.95048443395121	0.814490967873335\\
0.963458378673011	0.719869689937434\\
0.974527873505334	0.622071335778057\\
0.983647431519515	0.520298305594284\\
0.990779578495533	0.413287949972384\\
0.995895006911623	0.298774685976662\\
0.998972696375168	0.17159229222214\\
1	nan\\
};
\addplot[only marks, mark=+, mark options={}, mark size=1.5000pt, draw=mycolor2] table[row sep=crcr]{%
x	y\\
-1	inf\\
-0.963458378673011	25.4325895698062\\
-0.859174675048864	12.4562183433702\\
-0.702391671561197	8.01548430355851\\
-0.516025788785828	5.70774558770176\\
-0.327317472789346	4.24736022759455\\
-0.163849554869341	3.18904090286089\\
-0.0495155660487905	2.28268095528494\\
-0.00102730362483183	1.01134572323787\\
0.0163525684804853	1.40102925680806\\
0.0992931890660217	1.88661452954064\\
0.240803715844737	2.01531864841986\\
0.42020005248331	1.93780610804775\\
0.611260466978157	1.73690382974825\\
0.786058330061085	1.45510441420349\\
0.91904405244592	1.09001734183116\\
0.990779578495533	0.569612315457443\\
};
\addplot [color=mycolor2, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
-1	inf\\
-0.998972696375168	153.590149599352\\
-0.995895006911623	76.7516630856399\\
-0.990779578495533	51.1195434279563\\
-0.983647431519515	38.2890191178416\\
-0.974527873505334	30.5791369306403\\
-0.963458378673011	25.4295799434315\\
-0.95048443395121	21.7430700802373\\
-0.935659352061695	18.9709687164606\\
-0.91904405244592	16.808476844296\\
-0.900706810933978	15.072715097544\\
-0.880722979184567	13.6473055333208\\
-0.859174675048864	12.4546624675329\\
-0.836150445130658	11.4410720911141\\
-0.811744900929367	10.5681664614114\\
-0.786058330061085	9.80780780946419\\
-0.759196284155263	9.13889112976002\\
-0.731269145120418	8.54527514804735\\
-0.702391671561197	8.01440282633591\\
-0.672682527210654	7.53635733338369\\
-0.642263793315516	7.10320103067894\\
-0.611260466978157	6.70850309187572\\
-0.57979994751669	6.34699568458694\\
-0.548011512953841	6.01431952599741\\
-0.516025788785828	5.70683267243372\\
-0.483974211214172	5.42146475051224\\
-0.451988487046159	5.15560429079389\\
-0.42020005248331	4.90701045438143\\
-0.388739533021843	4.67374289784056\\
-0.357736206684484	4.45410520424898\\
-0.327317472789346	4.24659847131074\\
-0.297608328438803	4.04988245256765\\
-0.268730854879582	3.86274219731641\\
-0.240803715844737	3.68405849199913\\
-0.213941669938915	3.51278060472301\\
-0.188255099070633	3.34789988431265\\
-0.163849554869341	3.18842264763085\\
-0.140825324951136	3.03334044707434\\
-0.119277020815433	2.8815951224187\\
-0.0992931890660217	2.73203476225816\\
-0.0809559475540796	2.58335432989216\\
-0.0643406479383053	2.43401018119583\\
-0.0495155660487905	2.28208860171989\\
-0.0365416213269891	2.12508887908455\\
-0.0254721264946658	1.95953514573207\\
-0.0163525684804853	1.78020809774928\\
-0.00922042150446734	1.5784013075388\\
-0.00410499308837697	1.33705550947574\\
-0.00102730362483183	1.01101296105955\\
0	0\\
0	0\\
0.00102730362483183	0.816583356402874\\
0.00410499308837692	1.07461927263318\\
0.00922042150446734	1.2582527548733\\
0.0163525684804853	1.40302198182054\\
0.0254721264946657	1.52197327295849\\
0.0365416213269891	1.6215551098963\\
0.0495155660487904	1.70551304698228\\
0.0643406479383053	1.77627304954999\\
0.0809559475540797	1.83554184224156\\
0.0992931890660217	1.88460263169202\\
0.119277020815433	1.92447377404179\\
0.140825324951136	1.95599910530979\\
0.163849554869342	1.97990154375107\\
0.188255099070633	1.99681583963844\\
0.213941669938915	2.0073090140176\\
0.240803715844737	2.01189333637838\\
0.268730854879582	2.01103471032994\\
0.297608328438803	2.00515821506407\\
0.327317472789346	1.99465188699544\\
0.357736206684484	1.9798694194276\\
0.388739533021843	1.96113220228485\\
0.42020005248331	1.93873096004115\\
0.451988487046159	1.91292713981816\\
0.483974211214172	1.88395413252009\\
0.516025788785828	1.85201836477307\\
0.548011512953841	1.8173002698034\\
0.57979994751669	1.77995512542749\\
0.611260466978157	1.74011373293487\\
0.642263793315516	1.69788289873905\\
0.672682527210654	1.6533456686972\\
0.702391671561197	1.60656125053236\\
0.731269145120418	1.55756454010821\\
0.759196284155263	1.50636513884141\\
0.786058330061085	1.45294570707147\\
0.811744900929367	1.39725943351168\\
0.836150445130659	1.33922630031023\\
0.859174675048864	1.27872766311814\\
0.880722979184567	1.21559840333646\\
0.900706810933978	1.14961546550886\\
0.91904405244592	1.08048080930787\\
0.935659352061695	1.0077953552113\\
0.95048443395121	0.931017657411298\\
0.963458378673011	0.849395041841631\\
0.974527873505334	0.761841129823701\\
0.983647431519515	0.666697887756245\\
0.990779578495533	0.561211664654816\\
0.995895006911623	0.440134315551453\\
0.998972696375168	0.290425385598856\\
1	nan\\
};
\addplot[only marks, mark=+, mark options={}, mark size=1.5000pt, draw=mycolor3] table[row sep=crcr]{%
x	y\\
-1	inf\\
-0.963458378673011	23.6828966006309\\
-0.859174675048864	11.5298350912547\\
-0.702391671561197	7.33564751226695\\
-0.516025788785828	5.12402008031206\\
-0.327317472789346	3.6919686910526\\
-0.163849554869341	2.62083575001039\\
-0.0495155660487905	1.68161188516858\\
-0.00102730362483183	0.508062183097057\\
0.0163525684804853	0.674753634391383\\
0.0992931890660217	1.09867469130217\\
0.240803715844737	1.30567860705695\\
0.42020005248331	1.36417647996468\\
0.611260466978157	1.32024742684644\\
0.786058330061085	1.20170337051747\\
0.91904405244592	1.00534302674275\\
0.990779578495533	0.656730319140317\\
};
\addplot [color=mycolor3, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
-1	inf\\
-0.998972696375168	143.297310393988\\
-0.995895006911623	71.5970916304297\\
-0.990779578495533	47.6740835471917\\
-0.983647431519515	35.6953577212286\\
-0.974527873505334	28.494321710042\\
-0.963458378673011	23.6821055390042\\
-0.95048443395121	20.2349025709316\\
-0.935659352061695	17.640804666958\\
-0.91904405244592	15.6154138491549\\
-0.900706810933978	13.9880869052533\\
-0.880722979184567	12.6502283264511\\
-0.859174675048864	11.5294367066435\\
-0.836150445130658	10.5755834964122\\
-0.811744900929367	9.75285792078324\\
-0.786058330061085	9.03499383558795\\
-0.759196284155263	8.40228640679357\\
-0.731269145120418	7.83966160694508\\
-0.702391671561197	7.33538907706186\\
-0.672682527210654	6.88020129848126\\
-0.642263793315516	6.4666768360857\\
-0.611260466978157	6.08879959435255\\
-0.57979994751669	5.7416380417999\\
-0.548011512953841	5.42110784467119\\
-0.516025788785828	5.12379352704869\\
-0.483974211214172	4.84681256503963\\
-0.451988487046159	4.58771041340875\\
-0.42020005248331	4.3443783529787\\
-0.388739533021843	4.11498834239552\\
-0.357736206684484	3.89794063409806\\
-0.327317472789346	3.69182100859554\\
-0.297608328438803	3.49536524510617\\
-0.268730854879582	3.30742897778954\\
-0.240803715844737	3.12696144713361\\
-0.213941669938915	2.95298188239029\\
-0.188255099070633	2.78455736025553\\
-0.163849554869341	2.62078097487828\\
-0.140825324951136	2.46074899815418\\
-0.119277020815433	2.30353534260081\\
-0.0992931890660217	2.14816092844\\
-0.0809559475540796	1.99355422979484\\
-0.0643406479383053	1.83849675924994\\
-0.0495155660487905	1.68154226723368\\
-0.0365416213269891	1.52088790206614\\
-0.0254721264946658	1.35415130166708\\
-0.0163525684804853	1.17794477728369\\
-0.00922042150446734	0.986947171018784\\
-0.00410499308837697	0.771441091536362\\
-0.00102730362483183	0.508021406983535\\
0	0\\
0	0\\
0.00102730362483183	0.298178334627549\\
0.00410499308837692	0.450843230809809\\
0.00922042150446734	0.572672466894316\\
0.0163525684804853	0.67670621869456\\
0.0254721264946657	0.768060021999138\\
0.0365416213269891	0.849353027808928\\
0.0495155660487904	0.922137663774438\\
0.0643406479383053	0.987432765202483\\
0.0809559475540797	1.04596360398384\\
0.0992931890660217	1.09828343971667\\
0.119277020815433	1.14483996924445\\
0.140825324951136	1.18601347131162\\
0.163849554869342	1.22213932594728\\
0.188255099070633	1.25352145501198\\
0.213941669938915	1.28044030524765\\
0.240803715844737	1.3031574883382\\
0.268730854879582	1.32191836364428\\
0.297608328438803	1.33695336702724\\
0.327317472789346	1.34847859504798\\
0.357736206684484	1.35669596751635\\
0.388739533021843	1.36179316995461\\
0.42020005248331	1.36394349686069\\
0.451988487046159	1.36330566238642\\
0.483974211214172	1.36002360824231\\
0.516025788785828	1.35422631343215\\
0.548011512953841	1.34602759275134\\
0.57979994751669	1.33552585789292\\
0.611260466978157	1.32280380417997\\
0.642263793315516	1.30792797539576\\
0.672682527210654	1.29094814697738\\
0.702391671561197	1.27189645179306\\
0.731269145120418	1.2507861500208\\
0.759196284155263	1.22760991124714\\
0.786058330061085	1.20233742657839\\
0.811744900929367	1.17491209118683\\
0.836150445130659	1.14524637619473\\
0.859174675048864	1.11321531310168\\
0.880722979184567	1.0786471892945\\
0.900706810933978	1.04130999521655\\
0.91904405244592	1.00089116394354\\
0.935659352061695	0.956966260837861\\
0.95048443395121	0.908948515190518\\
0.963458378673011	0.856002980385285\\
0.974527873505334	0.79688997314353\\
0.983647431519515	0.729651481271562\\
0.990779578495533	0.650894133137583\\
0.995895006911623	0.553778873230362\\
0.998972696375168	0.419837372257261\\
1	nan\\
};
\addplot[only marks, mark=+, mark options={}, mark size=1.5000pt, draw=mycolor4] table[row sep=crcr]{%
x	y\\
-1	inf\\
-0.963458378673011	22.0547135173933\\
-0.859174675048864	10.6729322756161\\
-0.702391671561197	6.71387852187504\\
-0.516025788785828	4.60030428067965\\
-0.327317472789346	3.20946597797844\\
-0.163849554869341	2.15409677954028\\
-0.0495155660487905	1.23896482905284\\
-0.00102730362483183	0.255263275297174\\
0.0163525684804853	0.235042873981093\\
0.0992931890660217	0.462794335979167\\
0.240803715844737	0.611975950898549\\
0.42020005248331	0.694986883977138\\
0.611260466978157	0.726604283167945\\
0.786058330061085	0.718995359569588\\
0.91904405244592	0.672137677640998\\
0.990779578495533	0.54903143875343\\
};
\addplot [color=mycolor4, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
-1	inf\\
-0.998972696375168	133.694245495008\\
-0.995895006911623	66.7886964770571\\
-0.990779578495533	44.4608478412516\\
-0.983647431519515	33.2773884576414\\
-0.974527873505334	26.5516443958828\\
-0.963458378673011	22.0547143919851\\
-0.95048443395121	18.8313462884551\\
-0.935659352061695	16.4039060919303\\
-0.91904405244592	14.5070342743832\\
-0.900706810933978	12.9815082420554\\
-0.880722979184567	11.7259979503372\\
-0.859174675048864	10.6729436561623\\
-0.836150445130658	9.7755669572654\\
-0.811744900929367	9.00044846665685\\
-0.786058330061085	8.32307435004397\\
-0.759196284155263	7.72505283840074\\
-0.731269145120418	7.19231306735078\\
-0.702391671561197	6.71390421443026\\
-0.672682527210654	6.28117375723871\\
-0.642263793315516	5.88719214362011\\
-0.611260466978157	5.52634171773511\\
-0.57979994751669	5.19401761735864\\
-0.548011512953841	4.88640653967945\\
-0.516025788785828	4.60032063575997\\
-0.483974211214172	4.3330710650487\\
-0.451988487046159	4.08237049435347\\
-0.42020005248331	3.84625699278424\\
-0.388739533021843	3.62303392124432\\
-0.357736206684484	3.41122189311077\\
-0.327317472789346	3.20951991378186\\
-0.297608328438803	3.01677353350098\\
-0.268730854879582	2.83194836319176\\
-0.240803715844737	2.65410766769721\\
-0.213941669938915	2.48239300399259\\
-0.188255099070633	2.31600703739238\\
-0.163849554869341	2.15419775774946\\
-0.140825324951136	1.99624332895344\\
-0.119277020815433	1.84143672139379\\
-0.0992931890660217	1.68906905513238\\
-0.0809559475540796	1.53841012870225\\
-0.0643406479383053	1.38868372855857\\
-0.0495155660487905	1.23903357405246\\
-0.0365416213269891	1.08847212623294\\
-0.0254721264946658	0.935796304445253\\
-0.0163525684804853	0.779433539305996\\
-0.00922042150446734	0.61712107923988\\
-0.00410499308837697	0.445098467111633\\
-0.00102730362483183	0.255274422677089\\
0	0\\
0	0\\
0.00102730362483183	0.0787869491689154\\
0.00410499308837692	0.136867117120925\\
0.00922042150446734	0.188602460887195\\
0.0163525684804853	0.236177487253613\\
0.0254721264946657	0.280469689002393\\
0.0365416213269891	0.321919588278327\\
0.0495155660487904	0.360777224714515\\
0.0643406479383053	0.39719884732477\\
0.0809559475540797	0.431292091582147\\
0.0992931890660217	0.46313938569697\\
0.119277020815433	0.49281078955174\\
0.140825324951136	0.520371173357117\\
0.163849554869342	0.545884146649596\\
0.188255099070633	0.569414036120192\\
0.213941669938915	0.591026665840403\\
0.240803715844737	0.610789403299917\\
0.268730854879582	0.628770768119402\\
0.297608328438803	0.645039798066148\\
0.327317472789346	0.6596653005893\\
0.357736206684484	0.672715073026553\\
0.388739533021843	0.684255143124646\\
0.42020005248331	0.694349059091893\\
0.451988487046159	0.703057242302931\\
0.483974211214172	0.710436404160993\\
0.516025788785828	0.716539020160218\\
0.548011512953841	0.721412847845624\\
0.57979994751669	0.725100470277414\\
0.611260466978157	0.727638841987961\\
0.642263793315516	0.729058809495324\\
0.672682527210654	0.729384572337537\\
0.702391671561197	0.728633042229294\\
0.731269145120418	0.726813045811569\\
0.759196284155263	0.723924298316418\\
0.786058330061085	0.719956047750054\\
0.811744900929367	0.714885246042221\\
0.836150445130659	0.7086740349668\\
0.859174675048864	0.701266222634917\\
0.880722979184567	0.692582237955023\\
0.900706810933978	0.682511721843062\\
0.91904405244592	0.670902315662918\\
0.935659352061695	0.657542060825859\\
0.95048443395121	0.642130486420335\\
0.963458378673011	0.624228323205738\\
0.974527873505334	0.60316335384159\\
0.983647431519515	0.57783586738198\\
0.990779578495533	0.546256556880688\\
0.995895006911623	0.5041852945611\\
0.998972696375168	0.439167561141973\\
1	nan\\
};
\end{axis}
\end{tikzpicture}%

==> sections/pp-press-bet.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{tikzpicture}[%
trim axis left, trim axis right
]

\begin{axis}[%
width=0.951\fwidth,
height=\fheight,
at={(0\fwidth,0\fheight)},
scale only axis,
unbounded coords=jump,
xmin=-1,
xmax=1,
xlabel style={font=\color{white!15!black}},
xlabel={$x$},
ymin=0,
ymax=12,
ylabel style={font=\color{white!15!black}},
ylabel={$\left|p / \beta \right|$},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left
]
\addplot[only marks, mark=+, mark options={}, mark size=1.5000pt, draw=mycolor1] table[row sep=crcr]{%
x	y\\
-1	inf\\
-0.900706810933978	0.0133728464452352\\
-0.642263793315516	2.00984676411979\\
-0.327317472789346	2.79655741940187\\
-0.0809559475540796	2.74139672720683\\
0	0\\
0.0992931890660217	2.75818455104817\\
0.357736206684484	3.10358394268921\\
0.672682527210654	2.84377913126938\\
0.91904405244592	1.80597305073509\\
};
\addplot [color=mycolor1, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
-1	inf\\
-0.998972696375168	16.2931137661459\\
-0.995895006911623	7.8899854655962\\
-0.990779578495533	4.97599277674022\\
-0.983647431519515	3.43549525502162\\
-0.974527873505334	2.44574319460234\\
-0.963458378673011	1.73279438689419\\
-0.95048443395121	1.17950043337269\\
-0.935659352061695	0.727501800167967\\
-0.91904405244592	0.344558200458903\\
-0.900706810933978	0.0114796307218824\\
-0.880722979184567	0.283815023805236\\
-0.859174675048864	0.549269501492849\\
-0.836150445130658	0.790290897376556\\
-0.811744900929367	1.01066493929432\\
-0.786058330061085	1.21310561684055\\
-0.759196284155263	1.39959906051867\\
-0.731269145120418	1.57162631491885\\
-0.702391671561197	1.73031202215512\\
-0.672682527210654	1.87652622682389\\
-0.642263793315516	2.01095561984535\\
-0.611260466978157	2.13415431206365\\
-0.57979994751669	2.24658054751036\\
-0.548011512953841	2.34862352360233\\
-0.516025788785828	2.44062308139877\\
-0.483974211214172	2.52288412729046\\
-0.451988487046159	2.59568705398405\\
-0.42020005248331	2.65929502796238\\
-0.388739533021843	2.71395873213808\\
-0.357736206684484	2.7599189515421\\
-0.327317472789346	2.79740723709774\\
-0.297608328438803	2.82664475686071\\
-0.268730854879582	2.84783932872889\\
-0.240803715844737	2.86118050733979\\
-0.213941669938915	2.86683245145536\\
-0.188255099070633	2.86492409933884\\
-0.163849554869341	2.85553588492271\\
-0.140825324951136	2.83868176177847\\
-0.119277020815433	2.81428452770323\\
-0.0992931890660217	2.78214109627041\\
-0.0809559475540796	2.74187190861307\\
-0.0643406479383053	2.69284397077167\\
-0.0495155660487905	2.63404739316912\\
-0.0365416213269891	2.56388416406455\\
-0.0254721264946658	2.47977672353439\\
-0.0163525684804853	2.37736373134439\\
-0.00922042150446734	2.24859483930619\\
-0.00410499308837697	2.0761236881632\\
-0.00102730362483183	1.80874746324584\\
0	0\\
0	0\\
0.00102730362483183	1.72096737028991\\
0.00410499308837692	1.97793623328613\\
0.00922042150446734	2.14688301283354\\
0.0163525684804853	2.27667535536871\\
0.0254721264946657	2.38392153216747\\
0.0365416213269891	2.47634979955288\\
0.0495155660487904	2.55815079912385\\
0.0643406479383053	2.63179534154855\\
0.0809559475540797	2.6988032931516\\
0.0992931890660217	2.7601189595328\\
0.119277020815433	2.81631459501499\\
0.140825324951136	2.86771015381953\\
0.163849554869342	2.91444864685656\\
0.188255099070633	2.95654631576463\\
0.213941669938915	2.99392767849109\\
0.240803715844737	3.0264510166828\\
0.268730854879582	3.05392754264561\\
0.297608328438803	3.07613620808777\\
0.327317472789346	3.09283538915356\\
0.357736206684484	3.10377225145886\\
0.388739533021843	3.10869033512551\\
0.42020005248331	3.10733573315672\\
0.451988487046159	3.09946212777456\\
0.483974211214172	3.08483487600268\\
0.516025788785828	3.06323428444524\\
0.548011512953841	3.03445817571758\\
0.57979994751669	2.99832382015773\\
0.611260466978157	2.95466928284917\\
0.642263793315516	2.9033542151332\\
0.672682527210654	2.84426009965163\\
0.702391671561197	2.7772899365724\\
0.731269145120418	2.70236733374973\\
0.759196284155263	2.61943493214894\\
0.786058330061085	2.52845205552033\\
0.811744900929367	2.42939141314771\\
0.836150445130659	2.32223459523442\\
0.859174675048864	2.20696596284925\\
0.880722979184567	2.08356431412428\\
0.900706810933978	1.95199134223588\\
0.91904405244592	1.81217526568646\\
0.935659352061695	1.66398685561926\\
0.95048443395121	1.50720285764346\\
0.963458378673011	1.34144720526665\\
0.974527873505334	1.16609005822466\\
0.983647431519515	0.980058566956628\\
0.990779578495533	0.781436415846068\\
0.995895006911623	0.566445435334742\\
0.998972696375168	0.325849077838272\\
1	nan\\
};
\addplot[only marks, mark=+, mark options={}, mark size=1.5000pt, draw=mycolor2] table[row sep=crcr]{%
x	y\\
-1	inf\\
-0.900706810933978	1.51869883673933\\
-0.642263793315516	1.11997206742815\\
-0.327317472789346	2.00696422834201\\
-0.0809559475540796	1.8575332503805\\
0	0\\
0.0992931890660217	1.69372294505788\\
0.357736206684484	2.29173935496284\\
0.672682527210654	2.43591744268788\\
0.91904405244592	1.85262268653152\\
};
\addplot [color=mycolor2, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
-1	inf\\
-0.998972696375168	30.5602462024486\\
-0.995895006911623	15.03526757064\\
-0.990779578495533	9.75256494806958\\
-0.983647431519515	7.0316800163932\\
-0.974527873505334	5.33691174213309\\
-0.963458378673011	4.15667790788903\\
-0.95048443395121	3.27199359338598\\
-0.935659352061695	2.57358932405773\\
-0.91904405244592	2.00094919898841\\
-0.900706810933978	1.51792506959008\\
-0.880722979184567	1.10165116049168\\
-0.859174675048864	0.737000604359538\\
-0.836150445130658	0.413599848865728\\
-0.811744900929367	0.124122068094333\\
-0.786058330061085	0.136737219303864\\
-0.759196284155263	0.372900716794719\\
-0.731269145120418	0.587324066106544\\
-0.702391671561197	0.782272463313867\\
-0.672682527210654	0.959509969723867\\
-0.642263793315516	1.12043198589661\\
-0.611260466978157	1.26615974083621\\
-0.57979994751669	1.39760878285739\\
-0.548011512953841	1.51553927796826\\
-0.516025788785828	1.62059330668563\\
-0.483974211214172	1.71332267415519\\
-0.451988487046159	1.7942096494305\\
-0.42020005248331	1.86368231303791\\
-0.388739533021843	1.92212568670175\\
-0.357736206684484	1.96988946345754\\
-0.327317472789346	2.00729289746806\\
-0.297608328438803	2.03462721497182\\
-0.268730854879582	2.05215574498885\\
-0.240803715844737	2.06011181933655\\
-0.213941669938915	2.05869433507494\\
-0.188255099070633	2.04806068305028\\
-0.163849554869341	2.02831648655504\\
-0.140825324951136	1.9995012035128\\
-0.119277020815433	1.96156801653657\\
-0.0992931890660217	1.91435536562269\\
-0.0809559475540796	1.85754556626938\\
-0.0643406479383053	1.79060235281009\\
-0.0495155660487905	1.71267197248826\\
-0.0365416213269891	1.62241691016193\\
-0.0254721264946658	1.51771458948283\\
-0.0163525684804853	1.39505550337146\\
-0.00922042150446734	1.24816752067233\\
-0.00410499308837697	1.06415580395542\\
-0.00102730362483183	0.807771751567991\\
0	0\\
0	0\\
0.00102730362483183	0.654105564164309\\
0.00410499308837692	0.864106722793341\\
0.00922042150446734	1.01820382465773\\
0.0163525684804853	1.14536059849378\\
0.0254721264946657	1.25634651409709\\
0.0365416213269891	1.35649834070371\\
0.0495155660487904	1.44885988151075\\
0.0643406479383053	1.53530499856339\\
0.0809559475540797	1.61703150290707\\
0.0992931890660217	1.69481031077653\\
0.119277020815433	1.76912451763857\\
0.140825324951136	1.84025349385722\\
0.163849554869342	1.90832722162959\\
0.188255099070633	1.97336343542769\\
0.213941669938915	2.03529425375644\\
0.240803715844737	2.09398606038588\\
0.268730854879582	2.14925484516343\\
0.297608328438803	2.20087835669181\\
0.327317472789346	2.2486059243422\\
0.357736206684484	2.29216651137873\\
0.388739533021843	2.3312753783382\\
0.42020005248331	2.36563961919323\\
0.451988487046159	2.39496275561048\\
0.483974211214172	2.41894852126617\\
0.516025788785828	2.43730392934632\\
0.548011512953841	2.4497416861891\\
0.57979994751669	2.45598198864692\\
0.611260466978157	2.45575371933677\\
0.642263793315516	2.44879503014093\\
0.672682527210654	2.43485327772978\\
0.702391671561197	2.41368424265276\\
0.731269145120418	2.38505052180138\\
0.759196284155263	2.34871892706255\\
0.786058330061085	2.3044566418272\\
0.811744900929367	2.25202576723791\\
0.836150445130659	2.19117570738327\\
0.859174675048864	2.12163255493003\\
0.880722979184567	2.04308416994766\\
0.900706810933978	1.95515885214596\\
0.91904405244592	1.85739410902264\\
0.935659352061695	1.74918943323682\\
0.95048443395121	1.6297319170322\\
0.963458378673011	1.49787280333894\\
0.974527873505334	1.35190832005495\\
0.983647431519515	1.18915397509591\\
0.990779578495533	1.00500638827733\\
0.995895006911623	0.79043501966932\\
0.998972696375168	0.522467339026572\\
1	nan\\
};
\addplot[only marks, mark=+, mark options={}, mark size=1.5000pt, draw=mycolor3] table[row sep=crcr]{%
x	y\\
-1	inf\\
-0.900706810933978	2.80768143279004\\
-0.642263793315516	0.373250989904554\\
-0.327317472789346	1.37582213097943\\
-0.0809559475540796	1.23426383455535\\
0	0\\
0.0992931890660217	0.877567494462047\\
0.357736206684484	1.43420132330692\\
0.672682527210654	1.773557687016\\
0.91904405244592	1.61778908278378\\
};
\addplot [color=mycolor3, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
-1	inf\\
-0.998972696375168	42.8419832717999\\
-0.995895006911623	21.1852219228381\\
-0.990779578495533	13.8626499190132\\
-0.983647431519515	10.1248965347968\\
-0.974527873505334	7.8224855460347\\
-0.963458378673011	6.23924912886919\\
-0.95048443395121	5.06852811653768\\
-0.935659352061695	4.15722059766224\\
-0.91904405244592	3.42046353013903\\
-0.900706810933978	2.80750431382074\\
-0.880722979184567	2.28618695052124\\
-0.859174675048864	1.83519434127642\\
-0.836150445130658	1.43987040055297\\
-0.811744900929367	1.08983214213611\\
-0.786058330061085	0.777536481602895\\
-0.759196284155263	0.497384133690452\\
-0.731269145120418	0.245139516482533\\
-0.702391671561197	0.0175438414459233\\
-0.672682527210654	0.187949711756485\\
-0.642263793315516	0.373361390370007\\
-0.611260466978157	0.540317232666431\\
-0.57979994751669	0.690145193964519\\
-0.548011512953841	0.823945979425638\\
-0.516025788785828	0.942645872563065\\
-0.483974211214172	1.04703650745975\\
-0.451988487046159	1.1378050006236\\
-0.42020005248331	1.21555683515608\\
-0.388739533021843	1.2808331930637\\
-0.357736206684484	1.33412394754509\\
-0.327317472789346	1.37587718349277\\
-0.297608328438803	1.40650586369518\\
-0.268730854879582	1.42639206779779\\
-0.240803715844737	1.43588907722051\\
-0.213941669938915	1.43532144245526\\
-0.188255099070633	1.4249830304561\\
-0.163849554869341	1.40513288627095\\
-0.140825324951136	1.37598852141968\\
-0.119277020815433	1.33771590681208\\
-0.0992931890660217	1.29041490069617\\
-0.0809559475540796	1.23409788918291\\
-0.0643406479383053	1.16865765875235\\
-0.0495155660487905	1.09381706986653\\
-0.0365416213269891	1.0090458216482\\
-0.0254721264946658	0.913412797917979\\
-0.0163525684804853	0.805298921461819\\
-0.00922042150446734	0.681762950793714\\
-0.00410499308837697	0.536842003726607\\
-0.00102730362483183	0.355093092655588\\
0	0\\
0	0\\
0.00102730362483183	0.209031153923294\\
0.00410499308837692	0.317440969913282\\
0.00922042150446734	0.40615100835479\\
0.0163525684804853	0.484760237868565\\
0.0254721264946657	0.557206137435255\\
0.0365416213269891	0.625583856181375\\
0.0495155660487904	0.691156533038807\\
0.0643406479383053	0.754734999550378\\
0.0809559475540797	0.816851497456276\\
0.0992931890660217	0.877850473029537\\
0.119277020815433	0.937941079313026\\
0.140825324951136	0.99723016241202\\
0.163849554869342	1.05574451270787\\
0.188255099070633	1.11344682420883\\
0.213941669938915	1.17024775083513\\
0.240803715844737	1.22601540735947\\
0.268730854879582	1.28058310649414\\
0.297608328438803	1.33375581368067\\
0.327317472789346	1.38531562237522\\
0.357736206684484	1.43502644630488\\
0.388739533021843	1.48263805992872\\
0.42020005248331	1.52788957676762\\
0.451988487046159	1.57051242739399\\
0.483974211214172	1.61023287880134\\
0.516025788785828	1.64677412098585\\
0.548011512953841	1.67985793250722\\
0.57979994751669	1.70920592283855\\
0.611260466978157	1.73454033398951\\
0.642263793315516	1.7555843656382\\
0.672682527210654	1.77206196489083\\
0.702391671561197	1.78369699108283\\
0.731269145120418	1.79021162366873\\
0.759196284155263	1.791323820884\\
0.786058330061085	1.78674354831103\\
0.811744900929367	1.77616736289196\\
0.836150445130659	1.75927073057581\\
0.859174675048864	1.73569712406473\\
0.880722979184567	1.70504239855067\\
0.900706810933978	1.66683200163676\\
0.91904405244592	1.62048688612846\\
0.935659352061695	1.56527081414696\\
0.95048443395121	1.50020537558501\\
0.963458378673011	1.42392532989097\\
0.974527873505334	1.33441447214576\\
0.983647431519515	1.22847584234727\\
0.990779578495533	1.10051850807158\\
0.995895006911623	0.939150826044516\\
0.998972696375168	0.713292232382983\\
1	nan\\
};
\addplot[only marks, mark=+, mark options={}, mark size=1.5000pt, draw=mycolor4] table[row sep=crcr]{%
x	y\\
-1	inf\\
-0.900706810933978	3.90356391969\\
-0.642263793315516	0.248779074573602\\
-0.327317472789346	0.875232918055501\\
-0.0809559475540796	0.79866501122731\\
0	0\\
0.0992931890660217	0.324088588579087\\
0.357736206684484	0.643537412304661\\
0.672682527210654	0.929184910145692\\
0.91904405244592	1.01824986662084\\
};
\addplot [color=mycolor4, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
-1	inf\\
-0.998972696375168	53.3403536149872\\
-0.995895006911623	26.4413114534028\\
-0.990779578495533	17.3743913789583\\
-0.983647431519515	12.7667846094513\\
-0.974527873505334	9.94433091365982\\
-0.963458378673011	8.01597073500723\\
-0.95048443395121	6.60009374444839\\
-0.935659352061695	5.50612449009821\\
-0.91904405244592	4.62838300387106\\
-0.900706810933978	3.90362794458163\\
-0.880722979184567	3.2917570785308\\
-0.859174675048864	2.76615670390071\\
-0.836150445130658	2.30850448836278\\
-0.811744900929367	1.90579906889212\\
-0.786058330061085	1.54857731454343\\
-0.759196284155263	1.22979970677646\\
-0.731269145120418	0.944128787789545\\
-0.702391671561197	0.687447875217279\\
-0.672682527210654	0.456531582525348\\
-0.642263793315516	0.248815071966691\\
-0.611260466978157	0.0622291884225687\\
-0.57979994751669	0.104919428469883\\
-0.548011512953841	0.254036883090392\\
-0.516025788785828	0.386308296720224\\
-0.483974211214172	0.502747988187321\\
-0.451988487046159	0.604237833307376\\
-0.42020005248331	0.691556805438307\\
-0.388739533021843	0.765403838079778\\
-0.357736206684484	0.826415555665951\\
-0.327317472789346	0.875180001222956\\
-0.297608328438803	0.912247191516939\\
-0.268730854879582	0.938137113299701\\
-0.240803715844737	0.953345611984827\\
-0.213941669938915	0.958348497676701\\
-0.188255099070633	0.95360408816284\\
-0.163849554869341	0.939554310941892\\
-0.140825324951136	0.916624381890659\\
-0.119277020815433	0.885220946688287\\
-0.0992931890660217	0.8457283800426\\
-0.0809559475540796	0.798502627525465\\
-0.0643406479383053	0.743861426258303\\
-0.0495155660487905	0.682068695658814\\
-0.0365416213269891	0.61330873947798\\
-0.0254721264946658	0.537641060827081\\
-0.0163525684804853	0.454914383256109\\
-0.00922042150446734	0.364582531074045\\
-0.00410499308837697	0.265231954135839\\
-0.00102730362483183	0.15290240926651\\
0	0\\
0	0\\
0.00102730362483183	0.0473531076198199\\
0.00410499308837692	0.0826821088423628\\
0.00922042150446734	0.114900470718477\\
0.0163525684804853	0.145568600886032\\
0.0254721264946657	0.175425972797624\\
0.0365416213269891	0.204915216659603\\
0.0495155660487904	0.23433042332796\\
0.0643406479383053	0.263875339592085\\
0.0809559475540797	0.293690914895902\\
0.0992931890660217	0.323870218006113\\
0.119277020815433	0.354467476534477\\
0.140825324951136	0.38550414359749\\
0.163849554869342	0.416973362428524\\
0.188255099070633	0.448843517454131\\
0.213941669938915	0.481061231372567\\
0.240803715844737	0.51355399989316\\
0.268730854879582	0.54623256691166\\
0.297608328438803	0.578993094918658\\
0.327317472789346	0.611719159429294\\
0.357736206684484	0.644283582219926\\
0.388739533021843	0.676550110680857\\
0.42020005248331	0.708374946527286\\
0.451988487046159	0.739608124637106\\
0.483974211214172	0.770094740818245\\
0.516025788785828	0.799676025170131\\
0.548011512953841	0.828190254919594\\
0.57979994751669	0.85547349677762\\
0.611260466978157	0.881360163537783\\
0.642263793315516	0.905683362233755\\
0.672682527210654	0.928275000830998\\
0.702391671561197	0.94896560582373\\
0.731269145120418	0.967583782159935\\
0.759196284155263	0.983955216281381\\
0.786058330061085	0.997901077261818\\
0.811744900929367	1.00923560084974\\
0.836150445130659	1.01776253077011\\
0.859174675048864	1.02326991253605\\
0.880722979184567	1.02552243471508\\
0.900706810933978	1.02424998951216\\
0.91904405244592	1.01913017237995\\
0.935659352061695	1.00976061508115\\
0.95048443395121	0.995613323760249\\
0.963458378673011	0.975955002121016\\
0.974527873505334	0.949697512900543\\
0.983647431519515	0.915088287219323\\
0.990779578495533	0.868973775305082\\
0.995895006911623	0.804626794148325\\
0.998972696375168	0.702216939399686\\
1	nan\\
};
\end{axis}
\end{tikzpicture}%

==> sections/quadratic.tex <==
\section{Quadratic porosity relationship}

\textcolor{red}{SORRY I REALISED THAT THIS METHOD DOESN'T WORK DUE TO CROSS TERMS IN THE SQUARE. MAYBE IT IS A USEFUL START THOUGH.}

Now consider a porosity with quadratic dependence, such as that given in equation 10 of \cite{Bae2011}:

\begin{align*}
    -2 \vort(x) &= A w_s(x) + B w_s^2(x)
\end{align*}

where $A$ and $B$ are some constants that depend on the permeability and Ergun coefficient. 

Substituting the representation for the seepage velocity gives 

\begin{align*}
    -2 \vort(x) &= A \left( \frac{1}{2 \pi} \dashint_{-1}^1 \frac{\vort(t)}{x-t} \d t - U y^\prime(x) \right) + B \left( \frac{1}{2 \pi} \dashint_{-1}^1 \frac{\vort(t)}{x-t} \d t - U y^\prime(x) \right)^2 .
\end{align*}

We now seek a solution of the form

\begin{align*}
    \vort(x) &= \left( \sum_{n=1}^\infty \frac{s_n}{(1 + x)^{\alpha_n}}\right) \tilde{\vort}(x),
\end{align*}

where $\tilde{\vort}(x)$ is non-zero at $x=-1$.

Substitution of $\vort(x)$ into the quadratic singular integral equation, and letting $x \rightarrow -1$ gives

\begin{align*}
    &-2 \left( \sum_{n=1}^\infty \frac{s_n}{(1 + x)^{\alpha_n}}\right) \tilde{\vort}(-1) = A \left( \sum_{n=1}^\infty s_n \frac{\cot(\pi \alpha_n)}{2 (1 + x)^{\alpha_n}} \tilde{\vort}(-1) \right) + B \left( \sum_{n=1}^\infty s_n \frac{\cot(\pi \alpha_n)}{2  (1 + x)^{\alpha_n}}\tilde{\vort}(-1)\right)^2. \\
    &=  A \left( \sum_{n=1}^\infty s_n \frac{\cot(\pi \alpha_n)}{2 (1 + x)^{\alpha_n}} \tilde{\vort}(-1) \right) + B \tilde{\vort}(-1)^2 \left( \sum_{n=1}^\infty s_n^2 \frac{\cot(\pi \alpha_n)^2}{4  (1 + x)^{2 \alpha_n}} + \sum_{k=2}^\infty \sum_{j=1}^\infty s_j  s_{j+k} \frac{\cot(\pi \alpha_j)\cot(\pi \alpha_{j+k})}{4  (1 + x)^{ \alpha_j + \alpha_{j+k}}} \right). \\
\end{align*}

Now we solve the linear system for the coefficients $s_n$ by matching singular powers of $(1+x)$. For example, for the square root power ($n=1$), we have 

\begin{align*}
    -2 \frac{s_1}{(1+x)^{\frac{1}{2}}} \tilde{\vort}(-1) &= B \cot(\pi/4)^2\frac{s_2^2}{2^2  (1 + x)^{\frac{1}{2}}}\tilde{\vort}^2(-1).
\end{align*}

WLOG we can set $s_1=1$ which allows us to find $s_2$.

\subsection{Second attempt}

Now consider the Darcy–Forchheimer law, which is valid for larger pore-scale Reynolds numbers \footnote{ \verb| https://en.wikipedia.org/wiki/Darcy%27s_law#Darcy%E2%80%93Forchheimer_law | }:

\begin{align}
    -2 \Delta \gamma(t) = - \frac{\mu}{k} w_s(t) - \frac{\rho}{k_1} w_s(t)^2
\end{align}

Now use 

\begin{align*}
    w_s(t) = w(t)-y_{c,\alpha}^\prime(t) = \frac{1}{2 \pi} \dashint_{-1}^{1} \frac{\gamma(\tau)}{\tau - t} \d \tau - y_{c,\alpha}^\prime(t) 
\end{align*}

To obtain 


\begin{align}
    -2 \frac{k}{\mu} \Delta \gamma(t) = - \left( \frac{1}{2 \pi} \dashint_{-1}^{1} \frac{\gamma(\tau)}{\tau - t} \d \tau - y_{c,\alpha}^\prime(t)  \right) - \frac{\rho k}{\mu k_1} \left( \frac{1}{2 \pi} \dashint_{-1}^{1} \frac{\gamma(\tau)}{\tau - t} \d \tau - y_{c,\alpha}^\prime(t)  \right)^2
\end{align}

For trailing edge, need to take cross terms from second integral too. [Actually do not because the constant term cancels with geometry]. What happens to the square terms? Can we ignore these because they are higher order zeros than the original terms? I think so... Don't want to give quadratic terms too much influence at the trailing edge...

At leading edge need to do square and quarter root expansion. Perhaps we should do this at the trailing edge too.

e.g. write 
\begin{align*}
    \gamma(t) &= \frac{\gamma_{1/2}(t)}{(1+t)^{1/2}} + \frac{\gamma_{1/4}(t)}{(1+t)^{1/4}} 
\end{align*}

Note that 

\begin{align*}
   \frac{1}{ \pi} \dashint_{-1}^1 \frac{\phi^\ast(t)}{(1-t)^\beta} \frac{\d t}{ (t-\tau) }\sim  - \frac{\cot(\beta \pi)}{2 \pi \i } \cdot \frac{\phi^\ast(t)}{(1+t)^\beta}\   + \Phi_{\beta}^\ast(t)
\end{align*}

So 

\begin{align*}
   \frac{1}{ \pi} \dashint_{-1}^1 \frac{\gamma_{1/2}(t)}{(1-t)^{1/2}  } \frac{\d t}{ (t-\tau) } &\sim  0  + \Phi_{1/2}^\ast(t)\\
   \frac{1}{ \pi} \dashint_{-1}^1 \frac{\gamma_{1/4}(t)}{(1-t)^{1/4} } \frac{\d t}{ (t-\tau) }&\sim  - \frac{\cot( \pi)/4}{2 \pi \i } \cdot \frac{\phi^\ast(t)}{(1+t)^{1/4}}\   + \Phi_{1/4}^\ast(t)
\end{align*}

So that 

\begin{align}
     \frac{1}{ \pi} \dashint_{-1}^1 {\gamma(t)}  \frac{\d t}{ (t-\tau) } &\sim    - \frac{\cot( \pi)/4}{2 \pi \i } \cdot \frac{\phi^\ast(\tau)}{(1+\tau)^{1/4}} +\Phi_{1/2}^\ast(\tau)  + \Phi_{1/4}^\ast(\tau) \\ 
\end{align}

and 

\begin{align}
     \frac{1}{ \pi} \dashint_{-1}^1 {\gamma(t)}  \frac{\d t}{ (t-\tau) } &\sim    - \frac{\cot( \pi)/4}{2 \pi \i } \cdot \frac{\phi^\ast(t)}{(1+t)^{1/4}} +\Phi_{1/2}^\ast(t)  + \Phi_{1/4}^\ast(t) \\ 
\end{align}

Is it enough to account for the biggest zero/ smallest singularity?

At the trailing edge there are no cross terms, so the cross term method is impossible?! There is no way to match 1/2 and 1/4 terms. But are there actually cross terms at the leading edge? Otherwise the method there will not work... Further investigation into cross-terms... d

==> sections/results-vortex-shedding.tex <==
\subsection{Vortex shedding}

The inflow conditions and motion of the aerofoil camberline determine the distribution of vorticity along the chord line. Since Kelvin's circulation theorem implies that the net circulation remains constant, the variation of the inflow conditions and camber line must also affect the strength of the unsteady wake. In turn, the wake induces a velocity on the aerofoil surface, which must be corrected by the vorticity distribution. Accordingly, the wake vorticity has a strong effect on the unsteay lift of the aerofoil.

Accordging 

The numerical scheme may be used to rapidly determine relevant aerodynamic transfer functions. The input of these transfer functions is the inflow conditions and aerofoil geometry, whilst the output is the aerofoil lift response. 

==> sections/steady.tex <==
 \section{Numerical method} \label{Sec:Steady}
%
In this section we present our new numerical method. We begin by demonstrating why a typical Chebyshev expansion is not valid for porous aerofoils, and continue by applying our new method to a steady porous aerofoil for continuous and discontinuous porosity distributions. Analytic solutions are available for this steady problem, which enables direct comparison for our numerical solution.

Adopting the analysis given in \cite{Hajian2017}, the dimensionless pressure jump $p$ along a porous aerofoil with camber line $z(x)$ is the solution to the singular integral equation
%
\begin{equation}\label{Eq:p_steady}
2\rho UC R(x)p(x)-\frac{1}{\pi}\dashint_{-1}^{1}\frac{p(t)}{t-x}\d t~= 4\frac{\d z}{\d x}(x), \qquad \qquad -1<x<1,
\end{equation}
%
where $\rho$, $U$ and $C$ represent the air density, mean flow velocity, and the porosity coefficient respectively. The solution to equation \eqref{Eq:p_steady} is the focus of the present research. We also enforce that our solution must satisfy a Kutta condition, namely that the pressure jump must vanish at the trailing-edge. We note that analytic solutions to \eqref{Eq:p_steady} are available \cite{Hajian2017}, but we seek to develop a numerical solution that can be extended to the unsteady scenario.
%
%This equation can be solved by typical singular integral equation methods \cite{NIM}.  However, in this note we seek an expansion in terms of orthogonal polynomials. This approach will permit extensions to multiple bodies and unsteady motions. We note that for a rigid body, a typical expansion of the vortex sheet (or pressure) is given by (Rienstra, 1992)
%
\input{sections/chebyshev-failure}
\input{sections/continuous-porosity-steady}
\input{sections/partially-porous-steady}

==> sections/validation.tex <==
\section{Validation}
%
In this section we present numerical validation of our new method. The convergence of the scheme is observed to be exponentially fast for all tested parameters. In contrast, the Chebyshev expansion approach only to the continuous porosity solution algebraically fast and did not converge to a solution at all for the piecewise-continuous porosity problem.
%
\subsection{Continuous porosity distributions}
%
If $\tilde{p}(x)$ is expressible as a polynomial of degree $n$, then the proposed solution method is exact with $n$ Jacobi polynomials. For example, consider a flat plate at angle of attack $\alpha^\star$ with constant porosity $\psi_0$. The exact solution is given by \cite[B2]{Hajian2017} as
%
\begin{align}
p(x) & = \frac{-4\alpha^\star}{\sqrt{1+\psi_0^2} } \left(\frac{1-x}{1+x}\right)^{\frac{1}{\pi} \cot^{-1}(\psi_0)}. \label{Eq:alphSol}
\end{align}
%
Conversely, our collocation scheme \eqref{Eq:presCoef2} yields 
%
\begin{align*}
p_0 f_0^{k,-k}(x_j) + \sum_{n=1}^N p_n f_{n-1}^{k,1-k} (x_j) =-4\alpha^\star, \qquad \qquad j = 1, \cdots, N+1.
\end{align*}
%
Noting that $f_0^{k,-k}(x)$ is constant and the matrix $M$ with entries $\{M\}_{n,j} = f_{n-1}^{k,1-k} (x_j)$ has linearly independent rows, we obtain
%
\begin{align*}
p_0 & = \frac{-4\alpha^\star}{\sqrt{1+\psi_0} },\\
p_n & = 0, \qquad \qquad \qquad n>0,
\end{align*}
%
and the analytic solution \eqref{Eq:alphSol} is recovered.
%
%
\iffalse
\begin{figure}
\centering
\setlength{\fheight}{5cm}
\setlength{\fwidth}{.6\linewidth}
\begin{subfigure}[t]{\linewidth}
\centering
\input{images/pp-aoa-val.tex}
\caption{Errors for a flat plate at angle of attack with uniform porosity using the new spectral Jacobi method.}
\end{subfigure}

\begin{subfigure}[t]{\linewidth}
\centering
\input{images/pp-cam-val.tex}
\caption{Errors for a parabolic aerofoil with uniform porosity using the new spectral Jacobi method.}

\end{subfigure}
\label{Fig:uniPorVal}
\caption{The test} 
\end{figure}

\fi

\subsection{Discontinuous porosity distribution}

%
Exact solutions (not requiring Cauchy principal value integrals) are available when the porosity is constant and the aerofoil geometry is simple. The pressure jump along a parabolic aerofoil at angle of attack $\alpha^\star$ with parabolic profile $\beta^\star$ is given by \cite{gil2} as
%
\begin{align}
p(x) & = \frac{2 \left(\alpha^\star  + \beta^\star(1+x-(1-c)\arctan(\psi_0)/\pi)\right) }{\sqrt{1 + H(x-c) \psi_0^2}}  \sqrt{\frac{1-x}{1+x}} \left| \frac{x-c}{1-x} \right|^{\arctan(\psi_0)/\pi}. \label{Eq:pExact}
\end{align}
%
We now investigate the convergence of our method to this solution. We consider the relative $\mathcal{L}^2$ error, which is defined as
%
\begin{align*}
\epsilon_n & = \sqrt{\frac{\int_{-1}^{1} \left|p(x) - p_n(x)\right|^2 \d x}{\int_{-1}^{1} \left|p(x)\right|^2 \d x}},
\end{align*}
%
where $p$ is the exact solution and $p_n$ is the approximation using $n$ Jacobi polynomials.

The error decays exponentially fast for a range of porosities, as illustrated in figures \ref{Fig:ppAoa}b and \ref{Fig:ppCam}b. The slope of the line appears to be the same regardless of the porosity. This trend can be attributed to the fact that the porosity effect on the solution behaviour at the endpoints is accurately captured in the parameter of the Jacobi polynomials.
%
\begin{figure}[!h]
\begin{subfigure}[t]{.49\linewidth}
\centering
\setlength{\fheight}{5cm}
\setlength{\fwidth}{.8\linewidth}
\input{images/pp-press-aoa.tex}
\caption{Pressure distribution}
\end{subfigure}
\hfill
\begin{subfigure}[t]{.49\linewidth}
\centering
\setlength{\fheight}{5cm}
\setlength{\fwidth}{.8\linewidth}
\input{images/pp-aoa-val.tex}
\caption{Error convergence}
\end{subfigure}
\caption{The pressure distribution and error convergence for a partially porous aerofoil at angle of attack \bm{$\alpha^\star$} and permeable-impermeable junction at $c=0$. The coloured lines correspond to \textcolor{matlab1}{\bm{$\alpha = 0.4$}}, \textcolor{matlab2}{\bm{$\alpha= 0.3$}}, \textcolor{matlab3}{\bm{$\alpha=0.2$}} and \textcolor{matlab4}{\bm{$\alpha = 0.1$}}, where smaller $\alpha$ indicates a higher porosity. Note that \bm{$\alpha$} is defined in \textbf{\eqref{Eq:ppAlphDef}}. In (a) the solid line represents the exact solution \eqref{Eq:pExact} and the crosses (\bm{$+$}) represent the numerical solution with 5 polynomials.}
\label{Fig:ppAoa}
\end{figure}

\begin{figure}
\begin{subfigure}[t]{.49\linewidth}
\centering
\setlength{\fheight}{5cm}
\setlength{\fwidth}{.8\linewidth}
\input{images/pp-press-bet.tex}
\caption{Pressure distribution}
\end{subfigure}
\hfill
\begin{subfigure}[t]{.49\linewidth}
\centering
\setlength{\fheight}{5cm}
\setlength{\fwidth}{.8\linewidth}
\input{images/pp-cam-val.tex}
\caption{Error convergence}
\end{subfigure}
\centering
\caption{The pressure distribution and error convergence for a partially porous aerofoil with parabolic camber \bm{$\beta^\star$} and permeable-impermeable junction at $c=0$. The coloured lines correspond to \textcolor{matlab1}{\bm{$\alpha = 0.4$}}, \textcolor{matlab2}{\bm{$\alpha= 0.3$}}, \textcolor{matlab3}{\bm{$\alpha=0.2$}} and \textcolor{matlab4}{\bm{$\alpha = 0.1$}} where smaller $\alpha$ indicates a higher porosity. In a) the solid line represents the exact solution \eqref{Eq:pExact} and the crosses (\bm{$+$}) represent the numerical solution with 5 polynomials.}
\label{Fig:ppCam}
\end{figure}

We note that the error convergence in figures \ref{Fig:ppAoa}b and \ref{Fig:ppCam}b is not exactly linear, but instead features a ``staircase'' pattern. This is not a numerical error, but is rather a feature of the physical system. Recall that partially porous aerofoils consist of an impermeable forward part and a permeable aft part. The number of polynomials approximating the forward part is given by $N_+$ and the number of polynomials approximating the aft part is given by $N_-$. The variable on the $x$-axis in figures \ref{Fig:ppAoa}b and \ref{Fig:ppCam}b is $n = N_+ + N_-$. When $n$ increases from odd to even, $N_+$ increases by $1$, whereas when $n$ increases from even to odd, $N_-$ increases by $1$. The shallow decrease in error is associated with an improved approximation along the permeable aft section, whereas the steep decrease in error is associated with an improved approximation along the impermeable forward section. Hence there are two gradients associated with the slopes in figures \ref{Fig:ppAoa}b and \ref{Fig:ppCam}b.

\iffalse
These figures suggest that 
%
\begin{align*}
\epsilon_n &\sim \exp \left[-A n\right]
\end{align*}
%
for some constant $A$, although an explicit proof is not yet found.
\fi
